Derivation of Langevin Dynamics in a Nonzero Background Flow Field

We propose a derivation of a nonequilibrium Langevin dynamics for a large particle immersed in a background flow field. A single large particle is placed in an ideal gas heat bath composed of point particles that are distributed consistently with the background flow field and that interact with the large particle through elastic collisions. In the limit of small bath atom mass, the large particle dynamics converges in law to a stochastic dynamics. This derivation follows the ideas of [D. D\"urr, S. Goldstein, and J. L. Lebowitz, 1981 and 1983; P. Calderoni, D. D\"urr, and S. Kusuoka, 1989] and provides extensions to handle the nonzero background flow. The derived nonequilibrium Langevin dynamics is similar to the dynamics in [M. McPhie, et al., 2001]. Some numerical experiments illustrate the use of the obtained dynamic to simulate homogeneous liquid materials under flow.

==> figs/bath_nr1.tex <==
% GNUPLOT: plain TeX with Postscript
\begingroup
\catcode`\@=11\relax
\def\GNUPLOTspecial{%
  \def\do##1{\catcode`##1=12\relax}\dospecials
  \catcode`\{=1\catcode`\}=2\catcode\%=14\relax\special}%
%
\expandafter\ifx\csname GNUPLOTpicture\endcsname\relax
  \csname newdimen\endcsname\GNUPLOTunit
  \gdef\GNUPLOTpicture(#1,#2){\vbox to#2\GNUPLOTunit\bgroup
    \def\put(##1,##2)##3{\unskip\raise##2\GNUPLOTunit
      \hbox to0pt{\kern##1\GNUPLOTunit ##3\hss}\ignorespaces}%
    \def\ljust##1{\vbox to0pt{\vss\hbox to0pt{##1\hss}\vss}}%
    \def\cjust##1{\vbox to0pt{\vss\hbox to0pt{\hss ##1\hss}\vss}}%
    \def\rjust##1{\vbox to0pt{\vss\hbox to0pt{\hss ##1}\vss}}%
    \def\stack##1{\let\\=\cr\tabskip=0pt\halign{\hfil ####\hfil\cr ##1\crcr}}%
    \def\lstack##1{\hbox to0pt{\vbox to0pt{\vss\stack{##1}}\hss}}%
    \def\cstack##1{\hbox to0pt{\hss\vbox to0pt{\vss\stack{##1}}\hss}}%
    \def\rstack##1{\hbox to0pt{\vbox to0pt{\stack{##1}\vss}\hss}}%
    \vss\hbox to#1\GNUPLOTunit\bgroup\ignorespaces}%
  \gdef\endGNUPLOTpicture{\hss\egroup\egroup}%
\fi
\GNUPLOTunit=0.0500bp
\GNUPLOTpicture(3960,2772)
  {\GNUPLOTspecial{"
%!PS-Adobe-2.0 EPSF-2.0
%%Title: bath_nr1.tex
%%Creator: gnuplot 4.5 patchlevel 0
%%CreationDate: Sun Sep 04 20:15:10 2011
%%DocumentFonts: 
%%BoundingBox: 0 0 198 138
%%EndComments
%%BeginProlog
/gnudict 256 dict def
gnudict begin
%
% The following true/false flags may be edited by hand if desired.
% The unit line width and grayscale image gamma correction may also be changed.
%
/Color true def
/Blacktext true def
/Solid false def
/Dashlength 1 def
/Landscape false def
/Level1 false def
/Rounded false def
/ClipToBoundingBox false def
/SuppressPDFMark false def
/TransparentPatterns false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/Gamma 1.0 def
%
/vshift -66 def
/dl1 {
  10.0 Dashlength mul mul
  Rounded { currentlinewidth 0.75 mul sub dup 0 le { pop 0.01 } if } if
} def
/dl2 {
  10.0 Dashlength mul mul
  Rounded { currentlinewidth 0.75 mul add } if
} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/doclip {
  ClipToBoundingBox {
    newpath 0 0 moveto 198 0 lineto 198 138 lineto 0 138 lineto closepath
    clip
  } if
} def
%
% Gnuplot Prolog Version 4.4 (January 2010)
%
%/SuppressPDFMark true def
%
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/N {newpath moveto} bind def
/Z {closepath} bind def
/C {setrgbcolor} bind def
/f {rlineto fill} bind def
/Gshow {show} def   % May be redefined later in the file to support UTF-8
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow {currentpoint stroke M 0 vshift R 
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/Rshow {currentpoint stroke M dup stringwidth pop neg vshift R
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/Cshow {currentpoint stroke M dup stringwidth pop -2 div vshift R 
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/UP {dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def} def
/DL {Color {setrgbcolor Solid {pop []} if 0 setdash}
 {pop pop pop 0 setgray Solid {pop []} if 0 setdash} ifelse} def
/BL {stroke userlinewidth 2 mul setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
/AL {stroke userlinewidth 2 div setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
/UL {dup gnulinewidth mul /userlinewidth exch def
	dup 1 lt {pop 1} if 10 mul /udl exch def} def
/PL {stroke userlinewidth setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
% Default Line colors
/LCw {1 1 1} def
/LCb {0 0 0} def
/LCa {0 0 0} def
/LC0 {1 0 0} def
/LC1 {0 1 0} def
/LC2 {0 0 1} def
/LC3 {1 0 1} def
/LC4 {0 1 1} def
/LC5 {1 1 0} def
/LC6 {0 0 0} def
/LC7 {1 0.3 0} def
/LC8 {0.5 0.5 0.5} def
% Default Line Types
/LTw {PL [] 1 setgray} def
/LTb {BL [] LCb DL} def
/LTa {AL [1 udl mul 2 udl mul] 0 setdash LCa setrgbcolor} def
/LT0 {PL [] LC0 DL} def
/LT1 {PL [4 dl1 2 dl2] LC1 DL} def
/LT2 {PL [2 dl1 3 dl2] LC2 DL} def
/LT3 {PL [1 dl1 1.5 dl2] LC3 DL} def
/LT4 {PL [6 dl1 2 dl2 1 dl1 2 dl2] LC4 DL} def
/LT5 {PL [3 dl1 3 dl2 1 dl1 3 dl2] LC5 DL} def
/LT6 {PL [2 dl1 2 dl2 2 dl1 6 dl2] LC6 DL} def
/LT7 {PL [1 dl1 2 dl2 6 dl1 2 dl2 1 dl1 2 dl2] LC7 DL} def
/LT8 {PL [2 dl1 2 dl2 2 dl1 2 dl2 2 dl1 2 dl2 2 dl1 4 dl2] LC8 DL} def
/Pnt {stroke [] 0 setdash gsave 1 setlinecap M 0 0 V stroke grestore} def
/Dia {stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt} def
/Pls {stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
 } def
/Box {stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt} def
/Crs {stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke} def
/TriU {stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt} def
/Star {2 copy Pls Crs} def
/BoxF {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath fill} def
/TriUF {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill} def
/TriD {stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt} def
/TriDF {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill} def
/Pent {stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt} def
/PentF {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore} def
/Circle {stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt} def
/CircleF {stroke [] 0 setdash hpt 0 360 arc fill} def
/C0 {BL [] 0 setdash 2 copy moveto vpt 90 450 arc} bind def
/C1 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C2 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C3 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C4 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 180 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C5 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc
	2 copy moveto
	2 copy vpt 180 270 arc closepath fill
	vpt 0 360 arc} bind def
/C6 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C7 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C8 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 270 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C9 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 270 450 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C10 {BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
	2 copy moveto
	2 copy vpt 90 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C11 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 180 arc closepath fill
	2 copy moveto
	2 copy vpt 270 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C12 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 180 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C13 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc closepath fill
	2 copy moveto
	2 copy vpt 180 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C14 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 360 arc closepath fill
	vpt 0 360 arc} bind def
/C15 {BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/Rec {newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
	neg 0 rlineto closepath} bind def
/Square {dup Rec} bind def
/Bsquare {vpt sub exch vpt sub exch vpt2 Square} bind def
/S0 {BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare} bind def
/S1 {BL [] 0 setdash 2 copy vpt Square fill Bsquare} bind def
/S2 {BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare} bind def
/S3 {BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare} bind def
/S4 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare} bind def
/S5 {BL [] 0 setdash 2 copy 2 copy vpt Square fill
	exch vpt sub exch vpt sub vpt Square fill Bsquare} bind def
/S6 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare} bind def
/S7 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
	2 copy vpt Square fill Bsquare} bind def
/S8 {BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare} bind def
/S9 {BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare} bind def
/S10 {BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
	Bsquare} bind def
/S11 {BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
	Bsquare} bind def
/S12 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare} bind def
/S13 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
	2 copy vpt Square fill Bsquare} bind def
/S14 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
	2 copy exch vpt sub exch vpt Square fill Bsquare} bind def
/S15 {BL [] 0 setdash 2 copy Bsquare fill Bsquare} bind def
/D0 {gsave translate 45 rotate 0 0 S0 stroke grestore} bind def
/D1 {gsave translate 45 rotate 0 0 S1 stroke grestore} bind def
/D2 {gsave translate 45 rotate 0 0 S2 stroke grestore} bind def
/D3 {gsave translate 45 rotate 0 0 S3 stroke grestore} bind def
/D4 {gsave translate 45 rotate 0 0 S4 stroke grestore} bind def
/D5 {gsave translate 45 rotate 0 0 S5 stroke grestore} bind def
/D6 {gsave translate 45 rotate 0 0 S6 stroke grestore} bind def
/D7 {gsave translate 45 rotate 0 0 S7 stroke grestore} bind def
/D8 {gsave translate 45 rotate 0 0 S8 stroke grestore} bind def
/D9 {gsave translate 45 rotate 0 0 S9 stroke grestore} bind def
/D10 {gsave translate 45 rotate 0 0 S10 stroke grestore} bind def
/D11 {gsave translate 45 rotate 0 0 S11 stroke grestore} bind def
/D12 {gsave translate 45 rotate 0 0 S12 stroke grestore} bind def
/D13 {gsave translate 45 rotate 0 0 S13 stroke grestore} bind def
/D14 {gsave translate 45 rotate 0 0 S14 stroke grestore} bind def
/D15 {gsave translate 45 rotate 0 0 S15 stroke grestore} bind def
/DiaE {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke} def
/BoxE {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke} def
/TriUE {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke} def
/TriDE {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke} def
/PentE {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore} def
/CircE {stroke [] 0 setdash 
  hpt 0 360 arc stroke} def
/Opaque {gsave closepath 1 setgray fill grestore 0 setgray closepath} def
/DiaW {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke} def
/BoxW {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke} def
/TriUW {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke} def
/TriDW {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke} def
/PentW {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore} def
/CircW {stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke} def
/BoxFill {gsave Rec 1 setgray fill grestore} def
/Density {
  /Fillden exch def
  currentrgbcolor
  /ColB exch def /ColG exch def /ColR exch def
  /ColR ColR Fillden mul Fillden sub 1 add def
  /ColG ColG Fillden mul Fillden sub 1 add def
  /ColB ColB Fillden mul Fillden sub 1 add def
  ColR ColG ColB setrgbcolor} def
/BoxColFill {gsave Rec PolyFill} def
/PolyFill {gsave Density fill grestore grestore} def
/h {rlineto rlineto rlineto gsave closepath fill grestore} bind def
%
% PostScript Level 1 Pattern Fill routine for rectangles
% Usage: x y w h s a XX PatternFill
%	x,y = lower left corner of box to be filled
%	w,h = width and height of box
%	  a = angle in degrees between lines and x-axis
%	 XX = 0/1 for no/yes cross-hatch
%
/PatternFill {gsave /PFa [ 9 2 roll ] def
  PFa 0 get PFa 2 get 2 div add PFa 1 get PFa 3 get 2 div add translate
  PFa 2 get -2 div PFa 3 get -2 div PFa 2 get PFa 3 get Rec
  gsave 1 setgray fill grestore clip
  currentlinewidth 0.5 mul setlinewidth
  /PFs PFa 2 get dup mul PFa 3 get dup mul add sqrt def
  0 0 M PFa 5 get rotate PFs -2 div dup translate
  0 1 PFs PFa 4 get div 1 add floor cvi
	{PFa 4 get mul 0 M 0 PFs V} for
  0 PFa 6 get ne {
	0 1 PFs PFa 4 get div 1 add floor cvi
	{PFa 4 get mul 0 2 1 roll M PFs 0 V} for
 } if
  stroke grestore} def
%
/languagelevel where
 {pop languagelevel} {1} ifelse
 2 lt
	{/InterpretLevel1 true def}
	{/InterpretLevel1 Level1 def}
 ifelse
%
% PostScript level 2 pattern fill definitions
%
/Level2PatternFill {
/Tile8x8 {/PaintType 2 /PatternType 1 /TilingType 1 /BBox [0 0 8 8] /XStep 8 /YStep 8}
	bind def
/KeepColor {currentrgbcolor [/Pattern /DeviceRGB] setcolorspace} bind def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 8 8 L 0 8 M 8 0 L stroke} 
>> matrix makepattern
/Pat1 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 8 8 L 0 8 M 8 0 L stroke
	0 4 M 4 8 L 8 4 L 4 0 L 0 4 L stroke}
>> matrix makepattern
/Pat2 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 0 8 L
	8 8 L 8 0 L 0 0 L fill}
>> matrix makepattern
/Pat3 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -4 8 M 8 -4 L
	0 12 M 12 0 L stroke}
>> matrix makepattern
/Pat4 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -4 0 M 8 12 L
	0 -4 M 12 8 L stroke}
>> matrix makepattern
/Pat5 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -2 8 M 4 -4 L
	0 12 M 8 -4 L 4 12 M 10 0 L stroke}
>> matrix makepattern
/Pat6 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -2 0 M 4 12 L
	0 -4 M 8 12 L 4 -4 M 10 8 L stroke}
>> matrix makepattern
/Pat7 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 8 -2 M -4 4 L
	12 0 M -4 8 L 12 4 M 0 10 L stroke}
>> matrix makepattern
/Pat8 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 -2 M 12 4 L
	-4 0 M 12 8 L -4 4 M 8 10 L stroke}
>> matrix makepattern
/Pat9 exch def
/Pattern1 {PatternBgnd KeepColor Pat1 setpattern} bind def
/Pattern2 {PatternBgnd KeepColor Pat2 setpattern} bind def
/Pattern3 {PatternBgnd KeepColor Pat3 setpattern} bind def
/Pattern4 {PatternBgnd KeepColor Landscape {Pat5} {Pat4} ifelse setpattern} bind def
/Pattern5 {PatternBgnd KeepColor Landscape {Pat4} {Pat5} ifelse setpattern} bind def
/Pattern6 {PatternBgnd KeepColor Landscape {Pat9} {Pat6} ifelse setpattern} bind def
/Pattern7 {PatternBgnd KeepColor Landscape {Pat8} {Pat7} ifelse setpattern} bind def
} def
%
%
%End of PostScript Level 2 code
%
/PatternBgnd {
  TransparentPatterns {} {gsave 1 setgray fill grestore} ifelse
} def
%
% Substitute for Level 2 pattern fill codes with
% grayscale if Level 2 support is not selected.
%
/Level1PatternFill {
/Pattern1 {0.250 Density} bind def
/Pattern2 {0.500 Density} bind def
/Pattern3 {0.750 Density} bind def
/Pattern4 {0.125 Density} bind def
/Pattern5 {0.375 Density} bind def
/Pattern6 {0.625 Density} bind def
/Pattern7 {0.875 Density} bind def
} def
%
% Now test for support of Level 2 code
%
Level1 {Level1PatternFill} {Level2PatternFill} ifelse
%
/Symbol-Oblique /Symbol findfont [1 0 .167 1 0 0] makefont
dup length dict begin {1 index /FID eq {pop pop} {def} ifelse} forall
currentdict end definefont pop
Level1 SuppressPDFMark or 
{} {
/SDict 10 dict def
systemdict /pdfmark known not {
  userdict /pdfmark systemdict /cleartomark get put
} if
SDict begin [
  /Title (bath_nr1.tex)
  /Subject (gnuplot plot)
  /Creator (gnuplot 4.5 patchlevel 0)
  /Author (Matt)
%  /Producer (gnuplot)
%  /Keywords ()
  /CreationDate (Sun Sep 04 20:15:10 2011)
  /DOCINFO pdfmark
end
} ifelse
end
%%EndProlog
gnudict begin
gsave
doclip
0 0 translate
0.050 0.050 scale
0 setgray
newpath
1.000 UL
LTb
1.000 UP
1.000 UL
LTb
1.000 UL
LT0
LCa setrgbcolor
1.000 UL
LT0
LCa setrgbcolor
gsave 2115 1386 N -1 8 V 0 9 V -2 8 V -1 9 V -2 8 V -3 8 V -2 9 V -4 8 V -3 7 V -5 8 V -4 7 V -5 7 V -5 7 V -6 7 V -6 6 V -6 6 V -7 6 V -7 5 V -7 5 V -7 4 V -8 5 V -7 3 V -8 4 V -9 2 V -8 3 V -8 2 V -9 1 V -8 2 V -9 0 V -8 1 V -9 -1 V -9 0 V -8 -2 V -9 -1 V -8 -2 V -8 -3 V -9 -2 V -8 -4 V -7 -3 V -8 -5 V -7 -4 V -7 -5 V -7 -5 V -7 -6 V -6 -6 V -6 -6 V -6 -7 V -5 -7 V -5 -7 V -4 -7 V -5 -8 V -3 -7 V -4 -8 V -2 -9 V -3 -8 V -2 -8 V -1 -9 V -2 -8 V 0 -9 V 0 -8 V 0 -9 V 0 -9 V 2 -8 V 1 -9 V 2 -8 V 3 -8 V 2 -9 V 4 -8 V 3 -7 V 5 -8 V 4 -7 V 5 -7 V 5 -7 V 6 -7 V 6 -6 V 6 -6 V 7 -6 V 7 -5 V 7 -5 V 7 -4 V 8 -5 V 7 -3 V 8 -4 V 9 -2 V 8 -3 V 8 -2 V 9 -1 V 8 -2 V 9 0 V 8 0 V 9 0 V 9 0 V 8 2 V 9 1 V 8 2 V 8 3 V 9 2 V 8 4 V 7 3 V 8 5 V 7 4 V 7 5 V 7 5 V 7 6 V 2066 1269 L 6 6 V 6 7 V 5 7 V 5 7 V 4 7 V 5 8 V 3 7 V 4 8 V 2 9 V 3 8 V 2 8 V 1 9 V 2 8 V 0 9 V 1 8 V 1 PolyFill
2115 1386 M
-1 8 V
0 9 V
-2 8 V
-1 9 V
-2 8 V
-3 8 V
-2 9 V
-4 8 V
-3 7 V
-5 8 V
-4 7 V
-5 7 V
-5 7 V
-6 7 V
-6 6 V
-6 6 V
-7 6 V
-7 5 V
-7 5 V
-7 4 V
-8 5 V
-7 3 V
-8 4 V
-9 2 V
-8 3 V
-8 2 V
-9 1 V
-8 2 V
-9 0 V
-8 1 V
-9 -1 V
-9 0 V
-8 -2 V
-9 -1 V
-8 -2 V
-8 -3 V
-9 -2 V
-8 -4 V
-7 -3 V
-8 -5 V
-7 -4 V
-7 -5 V
-7 -5 V
-7 -6 V
-6 -6 V
-6 -6 V
-6 -7 V
-5 -7 V
-5 -7 V
-4 -7 V
-5 -8 V
-3 -7 V
-4 -8 V
-2 -9 V
-3 -8 V
-2 -8 V
-1 -9 V
-2 -8 V
0 -9 V
0 -8 V
0 -9 V
0 -9 V
2 -8 V
1 -9 V
2 -8 V
3 -8 V
2 -9 V
4 -8 V
3 -7 V
5 -8 V
4 -7 V
5 -7 V
5 -7 V
6 -7 V
6 -6 V
6 -6 V
7 -6 V
7 -5 V
7 -5 V
7 -4 V
8 -5 V
7 -3 V
8 -4 V
9 -2 V
8 -3 V
8 -2 V
9 -1 V
8 -2 V
9 0 V
8 0 V
9 0 V
9 0 V
8 2 V
9 1 V
8 2 V
8 3 V
9 2 V
8 4 V
7 3 V
8 5 V
7 4 V
7 5 V
7 5 V
7 6 V
stroke 2060 1263 M
6 6 V
6 6 V
6 7 V
5 7 V
5 7 V
4 7 V
5 8 V
3 7 V
4 8 V
2 9 V
3 8 V
2 8 V
1 9 V
2 8 V
0 9 V
1 8 V
stroke
3.000 UL
LTb
LCa setrgbcolor
3.000 UL
LTb
LCa setrgbcolor
305 2301 M
-5 6 V
2177 266 M
18 -1 V
-15 10 V
-36 7 R
51 -17 V
stroke
gsave [] 0 setdash
2177 266 M
18 -1 V
-15 10 V
stroke
grestore
1008 1608 M
7 23 V
-18 -16 V
-27 -52 R
45 68 V
stroke
gsave [] 0 setdash
1008 1608 M
7 23 V
-18 -16 V
stroke
grestore
454 928 M
422 908 L
38 1 V
84 37 R
422 908 L
stroke
gsave [] 0 setdash
454 928 M
422 908 L
38 1 V
stroke
grestore
3207 2244 M
37 38 V
-51 -15 V
-102 -78 R
153 93 V
stroke
gsave [] 0 setdash
3207 2244 M
37 38 V
-51 -15 V
stroke
grestore
2383 2273 M
-28 -22 V
35 5 V
76 42 R
-111 -47 V
stroke
gsave [] 0 setdash
2383 2273 M
-28 -22 V
35 5 V
stroke
grestore
1809 1632 M
-27 -11 V
29 -3 V
68 17 R
-97 -14 V
stroke
gsave [] 0 setdash
1809 1632 M
-27 -11 V
29 -3 V
stroke
grestore
713 1852 M
57 29 V
-64 2 V
560 1834 M
210 47 V
stroke
gsave [] 0 setdash
713 1852 M
57 29 V
-64 2 V
stroke
grestore
2990 2095 M
-6 -25 V
18 18 V
26 58 R
-44 -76 V
stroke
gsave [] 0 setdash
2990 2095 M
-6 -25 V
18 18 V
stroke
grestore
2512 1652 M
-12 17 V
2 -21 V
23 -45 R
-25 66 V
stroke
gsave [] 0 setdash
2512 1652 M
-12 17 V
2 -21 V
stroke
grestore
1607 1484 M
-16 -9 V
18 0 V
35 14 R
-53 -14 V
stroke
gsave [] 0 setdash
1607 1484 M
-16 -9 V
18 0 V
stroke
grestore
2251 502 M
-43 9 V
32 -29 V
99 -38 R
-131 67 V
stroke
gsave [] 0 setdash
2251 502 M
-43 9 V
32 -29 V
stroke
grestore
1434 1836 M
-12 -13 V
18 5 V
21 20 R
-39 -25 V
stroke
gsave [] 0 setdash
1434 1836 M
-12 -13 V
18 5 V
stroke
grestore
2484 792 M
61 -50 V
-27 74 V
2392 958 M
2545 742 L
stroke
gsave [] 0 setdash
2484 792 M
61 -50 V
-27 74 V
stroke
grestore
1006 1130 M
3 -20 V
7 19 V
-1 50 R
-6 -69 V
stroke
gsave [] 0 setdash
1006 1130 M
3 -20 V
7 19 V
stroke
grestore
1.000 UP
1.000 UL
LTb
stroke
grestore
end
showpage
  }}%
\endGNUPLOTpicture
\endgroup
\endinput


==> figs/bath_nr2.tex <==
% GNUPLOT: plain TeX with Postscript
\begingroup
\catcode`\@=11\relax
\def\GNUPLOTspecial{%
  \def\do##1{\catcode`##1=12\relax}\dospecials
  \catcode`\{=1\catcode`\}=2\catcode\%=14\relax\special}%
%
\expandafter\ifx\csname GNUPLOTpicture\endcsname\relax
  \csname newdimen\endcsname\GNUPLOTunit
  \gdef\GNUPLOTpicture(#1,#2){\vbox to#2\GNUPLOTunit\bgroup
    \def\put(##1,##2)##3{\unskip\raise##2\GNUPLOTunit
      \hbox to0pt{\kern##1\GNUPLOTunit ##3\hss}\ignorespaces}%
    \def\ljust##1{\vbox to0pt{\vss\hbox to0pt{##1\hss}\vss}}%
    \def\cjust##1{\vbox to0pt{\vss\hbox to0pt{\hss ##1\hss}\vss}}%
    \def\rjust##1{\vbox to0pt{\vss\hbox to0pt{\hss ##1}\vss}}%
    \def\stack##1{\let\\=\cr\tabskip=0pt\halign{\hfil ####\hfil\cr ##1\crcr}}%
    \def\lstack##1{\hbox to0pt{\vbox to0pt{\vss\stack{##1}}\hss}}%
    \def\cstack##1{\hbox to0pt{\hss\vbox to0pt{\vss\stack{##1}}\hss}}%
    \def\rstack##1{\hbox to0pt{\vbox to0pt{\stack{##1}\vss}\hss}}%
    \vss\hbox to#1\GNUPLOTunit\bgroup\ignorespaces}%
  \gdef\endGNUPLOTpicture{\hss\egroup\egroup}%
\fi
\GNUPLOTunit=0.0500bp
\GNUPLOTpicture(3960,2772)
  {\GNUPLOTspecial{"
%!PS-Adobe-2.0 EPSF-2.0
%%Title: bath_nr2.tex
%%Creator: gnuplot 4.5 patchlevel 0
%%CreationDate: Sun Sep 04 20:15:10 2011
%%DocumentFonts: 
%%BoundingBox: 0 0 198 138
%%EndComments
%%BeginProlog
/gnudict 256 dict def
gnudict begin
%
% The following true/false flags may be edited by hand if desired.
% The unit line width and grayscale image gamma correction may also be changed.
%
/Color true def
/Blacktext true def
/Solid false def
/Dashlength 1 def
/Landscape false def
/Level1 false def
/Rounded false def
/ClipToBoundingBox false def
/SuppressPDFMark false def
/TransparentPatterns false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/Gamma 1.0 def
%
/vshift -66 def
/dl1 {
  10.0 Dashlength mul mul
  Rounded { currentlinewidth 0.75 mul sub dup 0 le { pop 0.01 } if } if
} def
/dl2 {
  10.0 Dashlength mul mul
  Rounded { currentlinewidth 0.75 mul add } if
} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/doclip {
  ClipToBoundingBox {
    newpath 0 0 moveto 198 0 lineto 198 138 lineto 0 138 lineto closepath
    clip
  } if
} def
%
% Gnuplot Prolog Version 4.4 (January 2010)
%
%/SuppressPDFMark true def
%
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/N {newpath moveto} bind def
/Z {closepath} bind def
/C {setrgbcolor} bind def
/f {rlineto fill} bind def
/Gshow {show} def   % May be redefined later in the file to support UTF-8
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow {currentpoint stroke M 0 vshift R 
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/Rshow {currentpoint stroke M dup stringwidth pop neg vshift R
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/Cshow {currentpoint stroke M dup stringwidth pop -2 div vshift R 
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/UP {dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def} def
/DL {Color {setrgbcolor Solid {pop []} if 0 setdash}
 {pop pop pop 0 setgray Solid {pop []} if 0 setdash} ifelse} def
/BL {stroke userlinewidth 2 mul setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
/AL {stroke userlinewidth 2 div setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
/UL {dup gnulinewidth mul /userlinewidth exch def
	dup 1 lt {pop 1} if 10 mul /udl exch def} def
/PL {stroke userlinewidth setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
% Default Line colors
/LCw {1 1 1} def
/LCb {0 0 0} def
/LCa {0 0 0} def
/LC0 {1 0 0} def
/LC1 {0 1 0} def
/LC2 {0 0 1} def
/LC3 {1 0 1} def
/LC4 {0 1 1} def
/LC5 {1 1 0} def
/LC6 {0 0 0} def
/LC7 {1 0.3 0} def
/LC8 {0.5 0.5 0.5} def
% Default Line Types
/LTw {PL [] 1 setgray} def
/LTb {BL [] LCb DL} def
/LTa {AL [1 udl mul 2 udl mul] 0 setdash LCa setrgbcolor} def
/LT0 {PL [] LC0 DL} def
/LT1 {PL [4 dl1 2 dl2] LC1 DL} def
/LT2 {PL [2 dl1 3 dl2] LC2 DL} def
/LT3 {PL [1 dl1 1.5 dl2] LC3 DL} def
/LT4 {PL [6 dl1 2 dl2 1 dl1 2 dl2] LC4 DL} def
/LT5 {PL [3 dl1 3 dl2 1 dl1 3 dl2] LC5 DL} def
/LT6 {PL [2 dl1 2 dl2 2 dl1 6 dl2] LC6 DL} def
/LT7 {PL [1 dl1 2 dl2 6 dl1 2 dl2 1 dl1 2 dl2] LC7 DL} def
/LT8 {PL [2 dl1 2 dl2 2 dl1 2 dl2 2 dl1 2 dl2 2 dl1 4 dl2] LC8 DL} def
/Pnt {stroke [] 0 setdash gsave 1 setlinecap M 0 0 V stroke grestore} def
/Dia {stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt} def
/Pls {stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
 } def
/Box {stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt} def
/Crs {stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke} def
/TriU {stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt} def
/Star {2 copy Pls Crs} def
/BoxF {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath fill} def
/TriUF {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill} def
/TriD {stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt} def
/TriDF {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill} def
/Pent {stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt} def
/PentF {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore} def
/Circle {stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt} def
/CircleF {stroke [] 0 setdash hpt 0 360 arc fill} def
/C0 {BL [] 0 setdash 2 copy moveto vpt 90 450 arc} bind def
/C1 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C2 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C3 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C4 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 180 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C5 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc
	2 copy moveto
	2 copy vpt 180 270 arc closepath fill
	vpt 0 360 arc} bind def
/C6 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C7 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C8 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 270 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C9 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 270 450 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C10 {BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
	2 copy moveto
	2 copy vpt 90 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C11 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 180 arc closepath fill
	2 copy moveto
	2 copy vpt 270 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C12 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 180 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C13 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc closepath fill
	2 copy moveto
	2 copy vpt 180 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C14 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 360 arc closepath fill
	vpt 0 360 arc} bind def
/C15 {BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/Rec {newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
	neg 0 rlineto closepath} bind def
/Square {dup Rec} bind def
/Bsquare {vpt sub exch vpt sub exch vpt2 Square} bind def
/S0 {BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare} bind def
/S1 {BL [] 0 setdash 2 copy vpt Square fill Bsquare} bind def
/S2 {BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare} bind def
/S3 {BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare} bind def
/S4 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare} bind def
/S5 {BL [] 0 setdash 2 copy 2 copy vpt Square fill
	exch vpt sub exch vpt sub vpt Square fill Bsquare} bind def
/S6 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare} bind def
/S7 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
	2 copy vpt Square fill Bsquare} bind def
/S8 {BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare} bind def
/S9 {BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare} bind def
/S10 {BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
	Bsquare} bind def
/S11 {BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
	Bsquare} bind def
/S12 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare} bind def
/S13 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
	2 copy vpt Square fill Bsquare} bind def
/S14 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
	2 copy exch vpt sub exch vpt Square fill Bsquare} bind def
/S15 {BL [] 0 setdash 2 copy Bsquare fill Bsquare} bind def
/D0 {gsave translate 45 rotate 0 0 S0 stroke grestore} bind def
/D1 {gsave translate 45 rotate 0 0 S1 stroke grestore} bind def
/D2 {gsave translate 45 rotate 0 0 S2 stroke grestore} bind def
/D3 {gsave translate 45 rotate 0 0 S3 stroke grestore} bind def
/D4 {gsave translate 45 rotate 0 0 S4 stroke grestore} bind def
/D5 {gsave translate 45 rotate 0 0 S5 stroke grestore} bind def
/D6 {gsave translate 45 rotate 0 0 S6 stroke grestore} bind def
/D7 {gsave translate 45 rotate 0 0 S7 stroke grestore} bind def
/D8 {gsave translate 45 rotate 0 0 S8 stroke grestore} bind def
/D9 {gsave translate 45 rotate 0 0 S9 stroke grestore} bind def
/D10 {gsave translate 45 rotate 0 0 S10 stroke grestore} bind def
/D11 {gsave translate 45 rotate 0 0 S11 stroke grestore} bind def
/D12 {gsave translate 45 rotate 0 0 S12 stroke grestore} bind def
/D13 {gsave translate 45 rotate 0 0 S13 stroke grestore} bind def
/D14 {gsave translate 45 rotate 0 0 S14 stroke grestore} bind def
/D15 {gsave translate 45 rotate 0 0 S15 stroke grestore} bind def
/DiaE {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke} def
/BoxE {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke} def
/TriUE {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke} def
/TriDE {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke} def
/PentE {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore} def
/CircE {stroke [] 0 setdash 
  hpt 0 360 arc stroke} def
/Opaque {gsave closepath 1 setgray fill grestore 0 setgray closepath} def
/DiaW {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke} def
/BoxW {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke} def
/TriUW {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke} def
/TriDW {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke} def
/PentW {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore} def
/CircW {stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke} def
/BoxFill {gsave Rec 1 setgray fill grestore} def
/Density {
  /Fillden exch def
  currentrgbcolor
  /ColB exch def /ColG exch def /ColR exch def
  /ColR ColR Fillden mul Fillden sub 1 add def
  /ColG ColG Fillden mul Fillden sub 1 add def
  /ColB ColB Fillden mul Fillden sub 1 add def
  ColR ColG ColB setrgbcolor} def
/BoxColFill {gsave Rec PolyFill} def
/PolyFill {gsave Density fill grestore grestore} def
/h {rlineto rlineto rlineto gsave closepath fill grestore} bind def
%
% PostScript Level 1 Pattern Fill routine for rectangles
% Usage: x y w h s a XX PatternFill
%	x,y = lower left corner of box to be filled
%	w,h = width and height of box
%	  a = angle in degrees between lines and x-axis
%	 XX = 0/1 for no/yes cross-hatch
%
/PatternFill {gsave /PFa [ 9 2 roll ] def
  PFa 0 get PFa 2 get 2 div add PFa 1 get PFa 3 get 2 div add translate
  PFa 2 get -2 div PFa 3 get -2 div PFa 2 get PFa 3 get Rec
  gsave 1 setgray fill grestore clip
  currentlinewidth 0.5 mul setlinewidth
  /PFs PFa 2 get dup mul PFa 3 get dup mul add sqrt def
  0 0 M PFa 5 get rotate PFs -2 div dup translate
  0 1 PFs PFa 4 get div 1 add floor cvi
	{PFa 4 get mul 0 M 0 PFs V} for
  0 PFa 6 get ne {
	0 1 PFs PFa 4 get div 1 add floor cvi
	{PFa 4 get mul 0 2 1 roll M PFs 0 V} for
 } if
  stroke grestore} def
%
/languagelevel where
 {pop languagelevel} {1} ifelse
 2 lt
	{/InterpretLevel1 true def}
	{/InterpretLevel1 Level1 def}
 ifelse
%
% PostScript level 2 pattern fill definitions
%
/Level2PatternFill {
/Tile8x8 {/PaintType 2 /PatternType 1 /TilingType 1 /BBox [0 0 8 8] /XStep 8 /YStep 8}
	bind def
/KeepColor {currentrgbcolor [/Pattern /DeviceRGB] setcolorspace} bind def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 8 8 L 0 8 M 8 0 L stroke} 
>> matrix makepattern
/Pat1 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 8 8 L 0 8 M 8 0 L stroke
	0 4 M 4 8 L 8 4 L 4 0 L 0 4 L stroke}
>> matrix makepattern
/Pat2 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 0 8 L
	8 8 L 8 0 L 0 0 L fill}
>> matrix makepattern
/Pat3 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -4 8 M 8 -4 L
	0 12 M 12 0 L stroke}
>> matrix makepattern
/Pat4 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -4 0 M 8 12 L
	0 -4 M 12 8 L stroke}
>> matrix makepattern
/Pat5 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -2 8 M 4 -4 L
	0 12 M 8 -4 L 4 12 M 10 0 L stroke}
>> matrix makepattern
/Pat6 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -2 0 M 4 12 L
	0 -4 M 8 12 L 4 -4 M 10 8 L stroke}
>> matrix makepattern
/Pat7 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 8 -2 M -4 4 L
	12 0 M -4 8 L 12 4 M 0 10 L stroke}
>> matrix makepattern
/Pat8 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 -2 M 12 4 L
	-4 0 M 12 8 L -4 4 M 8 10 L stroke}
>> matrix makepattern
/Pat9 exch def
/Pattern1 {PatternBgnd KeepColor Pat1 setpattern} bind def
/Pattern2 {PatternBgnd KeepColor Pat2 setpattern} bind def
/Pattern3 {PatternBgnd KeepColor Pat3 setpattern} bind def
/Pattern4 {PatternBgnd KeepColor Landscape {Pat5} {Pat4} ifelse setpattern} bind def
/Pattern5 {PatternBgnd KeepColor Landscape {Pat4} {Pat5} ifelse setpattern} bind def
/Pattern6 {PatternBgnd KeepColor Landscape {Pat9} {Pat6} ifelse setpattern} bind def
/Pattern7 {PatternBgnd KeepColor Landscape {Pat8} {Pat7} ifelse setpattern} bind def
} def
%
%
%End of PostScript Level 2 code
%
/PatternBgnd {
  TransparentPatterns {} {gsave 1 setgray fill grestore} ifelse
} def
%
% Substitute for Level 2 pattern fill codes with
% grayscale if Level 2 support is not selected.
%
/Level1PatternFill {
/Pattern1 {0.250 Density} bind def
/Pattern2 {0.500 Density} bind def
/Pattern3 {0.750 Density} bind def
/Pattern4 {0.125 Density} bind def
/Pattern5 {0.375 Density} bind def
/Pattern6 {0.625 Density} bind def
/Pattern7 {0.875 Density} bind def
} def
%
% Now test for support of Level 2 code
%
Level1 {Level1PatternFill} {Level2PatternFill} ifelse
%
/Symbol-Oblique /Symbol findfont [1 0 .167 1 0 0] makefont
dup length dict begin {1 index /FID eq {pop pop} {def} ifelse} forall
currentdict end definefont pop
Level1 SuppressPDFMark or 
{} {
/SDict 10 dict def
systemdict /pdfmark known not {
  userdict /pdfmark systemdict /cleartomark get put
} if
SDict begin [
  /Title (bath_nr2.tex)
  /Subject (gnuplot plot)
  /Creator (gnuplot 4.5 patchlevel 0)
  /Author (Matt)
%  /Producer (gnuplot)
%  /Keywords ()
  /CreationDate (Sun Sep 04 20:15:10 2011)
  /DOCINFO pdfmark
end
} ifelse
end
%%EndProlog
gnudict begin
gsave
doclip
0 0 translate
0.050 0.050 scale
0 setgray
newpath
1.000 UL
LTb
1.000 UP
1.000 UL
LTb
1.000 UL
LT0
LCa setrgbcolor
1.000 UL
LT0
LCa setrgbcolor
gsave 2115 1386 N -1 8 V 0 9 V -2 8 V -1 9 V -2 8 V -3 8 V -2 9 V -4 8 V -3 7 V -5 8 V -4 7 V -5 7 V -5 7 V -6 7 V -6 6 V -6 6 V -7 6 V -7 5 V -7 5 V -7 4 V -8 5 V -7 3 V -8 4 V -9 2 V -8 3 V -8 2 V -9 1 V -8 2 V -9 0 V -8 1 V -9 -1 V -9 0 V -8 -2 V -9 -1 V -8 -2 V -8 -3 V -9 -2 V -8 -4 V -7 -3 V -8 -5 V -7 -4 V -7 -5 V -7 -5 V -7 -6 V -6 -6 V -6 -6 V -6 -7 V -5 -7 V -5 -7 V -4 -7 V -5 -8 V -3 -7 V -4 -8 V -2 -9 V -3 -8 V -2 -8 V -1 -9 V -2 -8 V 0 -9 V 0 -8 V 0 -9 V 0 -9 V 2 -8 V 1 -9 V 2 -8 V 3 -8 V 2 -9 V 4 -8 V 3 -7 V 5 -8 V 4 -7 V 5 -7 V 5 -7 V 6 -7 V 6 -6 V 6 -6 V 7 -6 V 7 -5 V 7 -5 V 7 -4 V 8 -5 V 7 -3 V 8 -4 V 9 -2 V 8 -3 V 8 -2 V 9 -1 V 8 -2 V 9 0 V 8 0 V 9 0 V 9 0 V 8 2 V 9 1 V 8 2 V 8 3 V 9 2 V 8 4 V 7 3 V 8 5 V 7 4 V 7 5 V 7 5 V 7 6 V 2066 1269 L 6 6 V 6 7 V 5 7 V 5 7 V 4 7 V 5 8 V 3 7 V 4 8 V 2 9 V 3 8 V 2 8 V 1 9 V 2 8 V 0 9 V 1 8 V 1 PolyFill
2115 1386 M
-1 8 V
0 9 V
-2 8 V
-1 9 V
-2 8 V
-3 8 V
-2 9 V
-4 8 V
-3 7 V
-5 8 V
-4 7 V
-5 7 V
-5 7 V
-6 7 V
-6 6 V
-6 6 V
-7 6 V
-7 5 V
-7 5 V
-7 4 V
-8 5 V
-7 3 V
-8 4 V
-9 2 V
-8 3 V
-8 2 V
-9 1 V
-8 2 V
-9 0 V
-8 1 V
-9 -1 V
-9 0 V
-8 -2 V
-9 -1 V
-8 -2 V
-8 -3 V
-9 -2 V
-8 -4 V
-7 -3 V
-8 -5 V
-7 -4 V
-7 -5 V
-7 -5 V
-7 -6 V
-6 -6 V
-6 -6 V
-6 -7 V
-5 -7 V
-5 -7 V
-4 -7 V
-5 -8 V
-3 -7 V
-4 -8 V
-2 -9 V
-3 -8 V
-2 -8 V
-1 -9 V
-2 -8 V
0 -9 V
0 -8 V
0 -9 V
0 -9 V
2 -8 V
1 -9 V
2 -8 V
3 -8 V
2 -9 V
4 -8 V
3 -7 V
5 -8 V
4 -7 V
5 -7 V
5 -7 V
6 -7 V
6 -6 V
6 -6 V
7 -6 V
7 -5 V
7 -5 V
7 -4 V
8 -5 V
7 -3 V
8 -4 V
9 -2 V
8 -3 V
8 -2 V
9 -1 V
8 -2 V
9 0 V
8 0 V
9 0 V
9 0 V
8 2 V
9 1 V
8 2 V
8 3 V
9 2 V
8 4 V
7 3 V
8 5 V
7 4 V
7 5 V
7 5 V
7 6 V
stroke 2060 1263 M
6 6 V
6 6 V
6 7 V
5 7 V
5 7 V
4 7 V
5 8 V
3 7 V
4 8 V
2 9 V
3 8 V
2 8 V
1 9 V
2 8 V
0 9 V
1 8 V
stroke
3.000 UL
LTb
LCa setrgbcolor
3.000 UL
LTb
LCa setrgbcolor
504 1125 M
-30 -8 V
30 -8 V
76 8 R
-106 0 V
stroke
gsave [] 0 setdash
504 1125 M
-30 -8 V
30 -8 V
stroke
grestore
2824 1900 M
27 7 V
-27 7 V
-69 -7 R
96 0 V
stroke
gsave [] 0 setdash
2824 1900 M
27 7 V
-27 7 V
stroke
grestore
3236 941 M
-37 -10 V
37 -10 V
92 10 R
-129 0 V
stroke
gsave [] 0 setdash
3236 941 M
-37 -10 V
37 -10 V
stroke
grestore
595 1984 M
37 9 V
-37 9 V
-91 -9 R
128 0 V
stroke
gsave [] 0 setdash
595 1984 M
37 9 V
-37 9 V
stroke
grestore
893 1211 M
18 4 V
-18 4 V
-28 -4 R
46 0 V
stroke
gsave [] 0 setdash
893 1211 M
18 4 V
-18 4 V
stroke
grestore
2965 2162 M
31 8 V
-31 8 V
-79 -8 R
110 0 V
stroke
gsave [] 0 setdash
2965 2162 M
31 8 V
-31 8 V
stroke
grestore
1021 668 M
-36 -9 V
36 -9 V
89 9 R
-125 0 V
stroke
gsave [] 0 setdash
1021 668 M
-36 -9 V
36 -9 V
stroke
grestore
2057 2142 M
18 4 V
-18 4 V
-38 -4 R
56 0 V
stroke
gsave [] 0 setdash
2057 2142 M
18 4 V
-18 4 V
stroke
grestore
2158 1294 M
-36 -9 V
36 -9 V
90 9 R
-126 0 V
stroke
gsave [] 0 setdash
2158 1294 M
-36 -9 V
36 -9 V
stroke
grestore
3162 1275 M
18 4 V
-18 4 V
-32 -4 R
50 0 V
stroke
gsave [] 0 setdash
3162 1275 M
18 4 V
-18 4 V
stroke
grestore
1277 329 M
-28 -7 V
28 -7 V
71 7 R
-99 0 V
stroke
gsave [] 0 setdash
1277 329 M
-28 -7 V
28 -7 V
stroke
grestore
1263 373 M
-58 -15 V
58 -15 V
144 15 R
-202 0 V
stroke
gsave [] 0 setdash
1263 373 M
-58 -15 V
58 -15 V
stroke
grestore
2595 2005 M
26 7 V
-26 7 V
-66 -7 R
92 0 V
stroke
gsave [] 0 setdash
2595 2005 M
26 7 V
-26 7 V
stroke
grestore
3414 2032 M
69 18 V
-69 18 V
-171 -18 R
240 0 V
stroke
gsave [] 0 setdash
3414 2032 M
69 18 V
-69 18 V
stroke
grestore
3415 1501 M
25 6 V
-25 6 V
-62 -6 R
87 0 V
stroke
gsave [] 0 setdash
3415 1501 M
25 6 V
-25 6 V
stroke
grestore
1902 2181 M
18 4 V
-18 4 V
-29 -4 R
47 0 V
stroke
gsave [] 0 setdash
1902 2181 M
18 4 V
-18 4 V
stroke
grestore
2514 2092 M
53 14 V
-53 14 V
-130 -14 R
183 0 V
stroke
gsave [] 0 setdash
2514 2092 M
53 14 V
-53 14 V
stroke
grestore
2621 2099 M
18 4 V
-18 4 V
-24 -4 R
42 0 V
stroke
gsave [] 0 setdash
2621 2099 M
18 4 V
-18 4 V
stroke
grestore
2135 2302 M
55 14 V
-55 14 V
-135 -14 R
190 0 V
stroke
gsave [] 0 setdash
2135 2302 M
55 14 V
-55 14 V
stroke
grestore
3281 2097 M
24 6 V
-24 6 V
-61 -6 R
85 0 V
stroke
gsave [] 0 setdash
3281 2097 M
24 6 V
-24 6 V
stroke
grestore
3527 1948 M
18 4 V
-18 4 V
-40 -4 R
58 0 V
stroke
gsave [] 0 setdash
3527 1948 M
18 4 V
-18 4 V
stroke
grestore
522 1812 M
-44 -11 V
44 -11 V
109 11 R
-153 0 V
stroke
gsave [] 0 setdash
522 1812 M
-44 -11 V
44 -11 V
stroke
grestore
928 1801 M
30 8 V
-30 8 V
-75 -8 R
105 0 V
stroke
gsave [] 0 setdash
928 1801 M
30 8 V
-30 8 V
stroke
grestore
1153 444 M
-54 -14 V
54 -14 V
135 14 R
-189 0 V
stroke
gsave [] 0 setdash
1153 444 M
-54 -14 V
54 -14 V
stroke
grestore
2728 1857 M
53 14 V
-53 14 V
-132 -14 R
185 0 V
stroke
gsave [] 0 setdash
2728 1857 M
53 14 V
-53 14 V
stroke
grestore
2161 2283 M
44 12 V
-44 12 V
-111 -12 R
155 0 V
stroke
gsave [] 0 setdash
2161 2283 M
44 12 V
-44 12 V
stroke
grestore
2146 2445 M
36 9 V
-36 9 V
-89 -9 R
125 0 V
stroke
gsave [] 0 setdash
2146 2445 M
36 9 V
-36 9 V
stroke
grestore
1875 1722 M
41 11 V
-41 11 V
-101 -11 R
142 0 V
stroke
gsave [] 0 setdash
1875 1722 M
41 11 V
-41 11 V
stroke
grestore
2996 943 M
18 4 V
-18 4 V
-9 -4 R
27 0 V
stroke
gsave [] 0 setdash
2996 943 M
18 4 V
-18 4 V
stroke
grestore
3563 769 M
-18 -4 V
18 -4 V
13 4 R
-31 0 V
stroke
gsave [] 0 setdash
3563 769 M
-18 -4 V
18 -4 V
stroke
grestore
1771 1078 M
18 4 V
-18 4 V
-30 -4 R
48 0 V
stroke
gsave [] 0 setdash
1771 1078 M
18 4 V
-18 4 V
stroke
grestore
3107 2363 M
51 13 V
-51 13 V
-125 -13 R
176 0 V
stroke
gsave [] 0 setdash
3107 2363 M
51 13 V
-51 13 V
stroke
grestore
3436 1214 M
-28 -7 V
28 -7 V
70 7 R
-98 0 V
stroke
gsave [] 0 setdash
3436 1214 M
-28 -7 V
28 -7 V
stroke
grestore
3303 261 M
-33 -9 V
33 -9 V
84 9 R
-117 0 V
stroke
gsave [] 0 setdash
3303 261 M
-33 -9 V
33 -9 V
stroke
grestore
1586 1188 M
18 4 V
-18 4 V
-14 -4 R
32 0 V
stroke
gsave [] 0 setdash
1586 1188 M
18 4 V
-18 4 V
stroke
grestore
2684 1207 M
18 4 V
-18 4 V
-34 -4 R
52 0 V
stroke
gsave [] 0 setdash
2684 1207 M
18 4 V
-18 4 V
stroke
grestore
3216 2466 M
46 12 V
-46 12 V
-115 -12 R
161 0 V
stroke
gsave [] 0 setdash
3216 2466 M
46 12 V
-46 12 V
stroke
grestore
3454 2220 M
145 0 V
2371 458 M
-62 -16 V
62 -16 V
152 16 R
-214 0 V
stroke
gsave [] 0 setdash
2371 458 M
-62 -16 V
62 -16 V
stroke
grestore
3304 2118 M
49 13 V
-49 13 V
-121 -13 R
170 0 V
stroke
gsave [] 0 setdash
3304 2118 M
49 13 V
-49 13 V
stroke
grestore
956 1886 M
18 4 V
-18 4 V
-32 -4 R
50 0 V
stroke
gsave [] 0 setdash
956 1886 M
18 4 V
-18 4 V
stroke
grestore
3032 1537 M
18 4 V
-18 4 V
-26 -4 R
44 0 V
stroke
gsave [] 0 setdash
3032 1537 M
18 4 V
-18 4 V
stroke
grestore
1445 2203 M
24 6 V
-24 6 V
-59 -6 R
83 0 V
stroke
gsave [] 0 setdash
1445 2203 M
24 6 V
-24 6 V
stroke
grestore
1138 1258 M
-18 -4 V
18 -4 V
33 4 R
-51 0 V
stroke
gsave [] 0 setdash
1138 1258 M
-18 -4 V
18 -4 V
stroke
grestore
3407 1669 M
-18 -4 V
18 -4 V
43 4 R
-61 0 V
stroke
gsave [] 0 setdash
3407 1669 M
-18 -4 V
18 -4 V
stroke
grestore
2942 2435 M
42 11 V
-42 11 V
-104 -11 R
146 0 V
stroke
gsave [] 0 setdash
2942 2435 M
42 11 V
-42 11 V
stroke
grestore
2264 485 M
-18 -4 V
18 -4 V
26 4 R
-44 0 V
stroke
gsave [] 0 setdash
2264 485 M
-18 -4 V
18 -4 V
stroke
grestore
1449 769 M
-24 -6 V
24 -6 V
60 6 R
-84 0 V
stroke
gsave [] 0 setdash
1449 769 M
-24 -6 V
24 -6 V
stroke
grestore
2349 2492 M
51 13 V
-51 13 V
-125 -13 R
176 0 V
stroke
gsave [] 0 setdash
2349 2492 M
51 13 V
-51 13 V
stroke
grestore
2241 1806 M
18 4 V
-18 4 V
-42 -4 R
60 0 V
stroke
gsave [] 0 setdash
2241 1806 M
18 4 V
-18 4 V
stroke
grestore
983 700 M
-28 -7 V
28 -7 V
72 7 R
-100 0 V
stroke
gsave [] 0 setdash
983 700 M
-28 -7 V
28 -7 V
stroke
grestore
2252 943 M
-54 -14 V
54 -14 V
133 14 R
-187 0 V
stroke
gsave [] 0 setdash
2252 943 M
-54 -14 V
54 -14 V
stroke
grestore
2928 2270 M
-18 -4 V
18 -4 V
21 4 R
-39 0 V
stroke
gsave [] 0 setdash
2928 2270 M
-18 -4 V
18 -4 V
stroke
grestore
1494 1839 M
56 15 V
-56 15 V
-140 -15 R
196 0 V
stroke
gsave [] 0 setdash
1494 1839 M
56 15 V
-56 15 V
stroke
grestore
746 593 M
703 582 L
43 -11 V
107 11 R
-150 0 V
stroke
gsave [] 0 setdash
746 593 M
703 582 L
43 -11 V
stroke
grestore
1316 899 M
-22 -6 V
22 -6 V
57 6 R
-79 0 V
stroke
gsave [] 0 setdash
1316 899 M
-22 -6 V
22 -6 V
stroke
grestore
3554 2413 M
45 0 V
1413 928 M
-24 -6 V
24 -6 V
62 6 R
-86 0 V
stroke
gsave [] 0 setdash
1413 928 M
-24 -6 V
24 -6 V
stroke
grestore
578 540 M
36 9 V
-36 9 V
-90 -9 R
126 0 V
stroke
gsave [] 0 setdash
578 540 M
36 9 V
-36 9 V
stroke
grestore
1891 970 M
18 4 V
-18 4 V
-12 -4 R
30 0 V
stroke
gsave [] 0 setdash
1891 970 M
18 4 V
-18 4 V
stroke
grestore
1952 737 M
-18 -4 V
18 -4 V
4 4 R
-22 0 V
stroke
gsave [] 0 setdash
1952 737 M
-18 -4 V
18 -4 V
stroke
grestore
1769 1506 M
-18 -4 V
18 -4 V
-15 4 R
-3 0 V
stroke
gsave [] 0 setdash
1769 1506 M
-18 -4 V
18 -4 V
stroke
grestore
675 1941 M
36 9 V
-36 9 V
-89 -9 R
125 0 V
stroke
gsave [] 0 setdash
675 1941 M
36 9 V
-36 9 V
stroke
grestore
795 426 M
756 416 L
39 -10 V
99 10 R
-138 0 V
stroke
gsave [] 0 setdash
795 426 M
756 416 L
39 -10 V
stroke
grestore
379 273 M
-21 -5 V
21 -5 V
53 5 R
-74 0 V
stroke
gsave [] 0 setdash
379 273 M
-21 -5 V
21 -5 V
stroke
grestore
2018 2467 M
55 14 V
-55 14 V
-135 -14 R
190 0 V
stroke
gsave [] 0 setdash
2018 2467 M
55 14 V
-55 14 V
stroke
grestore
1969 973 M
-18 -4 V
18 -4 V
24 4 R
-42 0 V
stroke
gsave [] 0 setdash
1969 973 M
-18 -4 V
18 -4 V
stroke
grestore
3279 1678 M
-18 -4 V
18 -4 V
11 4 R
-29 0 V
stroke
gsave [] 0 setdash
3279 1678 M
-18 -4 V
18 -4 V
stroke
grestore
1558 1490 M
18 4 V
-18 4 V
-21 -4 R
39 0 V
stroke
gsave [] 0 setdash
1558 1490 M
18 4 V
-18 4 V
stroke
grestore
3136 1056 M
-26 -7 V
26 -7 V
66 7 R
-92 0 V
stroke
gsave [] 0 setdash
3136 1056 M
-26 -7 V
26 -7 V
stroke
grestore
1909 642 M
-68 -18 V
68 -18 V
170 18 R
-238 0 V
stroke
gsave [] 0 setdash
1909 642 M
-68 -18 V
68 -18 V
stroke
grestore
775 1403 M
22 5 V
-22 5 V
-55 -5 R
77 0 V
stroke
gsave [] 0 setdash
775 1403 M
22 5 V
-22 5 V
stroke
grestore
1899 870 M
-71 -19 V
71 -19 V
175 19 R
-246 0 V
stroke
gsave [] 0 setdash
1899 870 M
-71 -19 V
71 -19 V
stroke
grestore
3442 1045 M
-18 -4 V
18 -4 V
14 4 R
-32 0 V
stroke
gsave [] 0 setdash
3442 1045 M
-18 -4 V
18 -4 V
stroke
grestore
2760 473 M
-33 -9 V
33 -9 V
83 9 R
-116 0 V
stroke
gsave [] 0 setdash
2760 473 M
-33 -9 V
33 -9 V
stroke
grestore
3269 2175 M
18 4 V
-18 4 V
-25 -4 R
43 0 V
stroke
gsave [] 0 setdash
3269 2175 M
18 4 V
-18 4 V
stroke
grestore
3213 1574 M
26 7 V
-26 7 V
-65 -7 R
91 0 V
stroke
gsave [] 0 setdash
3213 1574 M
26 7 V
-26 7 V
stroke
grestore
1401 440 M
-68 -18 V
68 -18 V
168 18 R
-236 0 V
stroke
gsave [] 0 setdash
1401 440 M
-68 -18 V
68 -18 V
stroke
grestore
3455 250 M
-23 -6 V
23 -6 V
58 6 R
-81 0 V
stroke
gsave [] 0 setdash
3455 250 M
-23 -6 V
23 -6 V
stroke
grestore
2370 2131 M
18 4 V
-18 4 V
-3 -4 R
21 0 V
stroke
gsave [] 0 setdash
2370 2131 M
18 4 V
-18 4 V
stroke
grestore
3137 426 M
-36 -9 V
36 -9 V
89 9 R
-125 0 V
stroke
gsave [] 0 setdash
3137 426 M
-36 -9 V
36 -9 V
stroke
grestore
640 547 M
591 534 L
49 -13 V
122 13 R
-171 0 V
stroke
gsave [] 0 setdash
640 547 M
591 534 L
49 -13 V
stroke
grestore
1594 2320 M
58 15 V
-58 15 V
-144 -15 R
202 0 V
stroke
gsave [] 0 setdash
1594 2320 M
58 15 V
-58 15 V
stroke
grestore
3064 1242 M
-18 -4 V
18 -4 V
28 4 R
-46 0 V
stroke
gsave [] 0 setdash
3064 1242 M
-18 -4 V
18 -4 V
stroke
grestore
2148 1898 M
18 4 V
-18 4 V
-28 -4 R
46 0 V
stroke
gsave [] 0 setdash
2148 1898 M
18 4 V
-18 4 V
stroke
grestore
3327 643 M
-18 -4 V
18 -4 V
13 4 R
-31 0 V
stroke
gsave [] 0 setdash
3327 643 M
-18 -4 V
18 -4 V
stroke
grestore
366 1064 M
-26 -7 V
26 -7 V
67 7 R
-93 0 V
stroke
gsave [] 0 setdash
366 1064 M
-26 -7 V
26 -7 V
stroke
grestore
450 1938 M
32 8 V
-32 8 V
-81 -8 R
113 0 V
stroke
gsave [] 0 setdash
450 1938 M
32 8 V
-32 8 V
stroke
grestore
2569 975 M
-18 -4 V
18 -4 V
44 4 R
-62 0 V
stroke
gsave [] 0 setdash
2569 975 M
-18 -4 V
18 -4 V
stroke
grestore
2005 2052 M
18 4 V
-18 4 V
-39 -4 R
57 0 V
stroke
gsave [] 0 setdash
2005 2052 M
18 4 V
-18 4 V
stroke
grestore
581 962 M
-26 -7 V
26 -7 V
66 7 R
-92 0 V
stroke
gsave [] 0 setdash
581 962 M
-26 -7 V
26 -7 V
stroke
grestore
1339 1663 M
27 7 V
-27 7 V
-69 -7 R
96 0 V
stroke
gsave [] 0 setdash
1339 1663 M
27 7 V
-27 7 V
stroke
grestore
1416 1604 M
20 5 V
-20 5 V
-50 -5 R
70 0 V
stroke
gsave [] 0 setdash
1416 1604 M
20 5 V
-20 5 V
stroke
grestore
338 1470 M
-18 -4 V
18 -4 V
2 4 R
-20 0 V
stroke
gsave [] 0 setdash
338 1470 M
-18 -4 V
18 -4 V
stroke
grestore
2439 1801 M
18 4 V
-18 4 V
5 -4 R
13 0 V
stroke
gsave [] 0 setdash
2439 1801 M
18 4 V
-18 4 V
stroke
grestore
1219 734 M
-18 -4 V
18 -4 V
18 4 R
-36 0 V
stroke
gsave [] 0 setdash
1219 734 M
-18 -4 V
18 -4 V
stroke
grestore
1814 790 M
-74 -19 V
74 -19 V
182 19 R
-256 0 V
stroke
gsave [] 0 setdash
1814 790 M
-74 -19 V
74 -19 V
stroke
grestore
2124 2240 M
18 4 V
-18 4 V
-10 -4 R
28 0 V
stroke
gsave [] 0 setdash
2124 2240 M
18 4 V
-18 4 V
stroke
grestore
1599 1540 M
41 11 V
-41 11 V
-102 -11 R
143 0 V
stroke
gsave [] 0 setdash
1599 1540 M
41 11 V
-41 11 V
stroke
grestore
2630 2509 M
26 7 V
-26 7 V
-65 -7 R
91 0 V
stroke
gsave [] 0 setdash
2630 2509 M
26 7 V
-26 7 V
stroke
grestore
1.000 UP
1.000 UL
LTb
stroke
grestore
end
showpage
  }}%
\endGNUPLOTpicture
\endgroup
\endinput


==> figs/bath_nr3.tex <==
% GNUPLOT: plain TeX with Postscript
\begingroup
\catcode`\@=11\relax
\def\GNUPLOTspecial{%
  \def\do##1{\catcode`##1=12\relax}\dospecials
  \catcode`\{=1\catcode`\}=2\catcode\%=14\relax\special}%
%
\expandafter\ifx\csname GNUPLOTpicture\endcsname\relax
  \csname newdimen\endcsname\GNUPLOTunit
  \gdef\GNUPLOTpicture(#1,#2){\vbox to#2\GNUPLOTunit\bgroup
    \def\put(##1,##2)##3{\unskip\raise##2\GNUPLOTunit
      \hbox to0pt{\kern##1\GNUPLOTunit ##3\hss}\ignorespaces}%
    \def\ljust##1{\vbox to0pt{\vss\hbox to0pt{##1\hss}\vss}}%
    \def\cjust##1{\vbox to0pt{\vss\hbox to0pt{\hss ##1\hss}\vss}}%
    \def\rjust##1{\vbox to0pt{\vss\hbox to0pt{\hss ##1}\vss}}%
    \def\stack##1{\let\\=\cr\tabskip=0pt\halign{\hfil ####\hfil\cr ##1\crcr}}%
    \def\lstack##1{\hbox to0pt{\vbox to0pt{\vss\stack{##1}}\hss}}%
    \def\cstack##1{\hbox to0pt{\hss\vbox to0pt{\vss\stack{##1}}\hss}}%
    \def\rstack##1{\hbox to0pt{\vbox to0pt{\stack{##1}\vss}\hss}}%
    \vss\hbox to#1\GNUPLOTunit\bgroup\ignorespaces}%
  \gdef\endGNUPLOTpicture{\hss\egroup\egroup}%
\fi
\GNUPLOTunit=0.0500bp
\GNUPLOTpicture(3960,2772)
  {\GNUPLOTspecial{"
%!PS-Adobe-2.0 EPSF-2.0
%%Title: bath_nr3.tex
%%Creator: gnuplot 4.5 patchlevel 0
%%CreationDate: Sun Sep 04 20:15:10 2011
%%DocumentFonts: 
%%BoundingBox: 0 0 198 138
%%EndComments
%%BeginProlog
/gnudict 256 dict def
gnudict begin
%
% The following true/false flags may be edited by hand if desired.
% The unit line width and grayscale image gamma correction may also be changed.
%
/Color true def
/Blacktext true def
/Solid false def
/Dashlength 1 def
/Landscape false def
/Level1 false def
/Rounded false def
/ClipToBoundingBox false def
/SuppressPDFMark false def
/TransparentPatterns false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/Gamma 1.0 def
%
/vshift -66 def
/dl1 {
  10.0 Dashlength mul mul
  Rounded { currentlinewidth 0.75 mul sub dup 0 le { pop 0.01 } if } if
} def
/dl2 {
  10.0 Dashlength mul mul
  Rounded { currentlinewidth 0.75 mul add } if
} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/doclip {
  ClipToBoundingBox {
    newpath 0 0 moveto 198 0 lineto 198 138 lineto 0 138 lineto closepath
    clip
  } if
} def
%
% Gnuplot Prolog Version 4.4 (January 2010)
%
%/SuppressPDFMark true def
%
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/N {newpath moveto} bind def
/Z {closepath} bind def
/C {setrgbcolor} bind def
/f {rlineto fill} bind def
/Gshow {show} def   % May be redefined later in the file to support UTF-8
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow {currentpoint stroke M 0 vshift R 
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/Rshow {currentpoint stroke M dup stringwidth pop neg vshift R
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/Cshow {currentpoint stroke M dup stringwidth pop -2 div vshift R 
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/UP {dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def} def
/DL {Color {setrgbcolor Solid {pop []} if 0 setdash}
 {pop pop pop 0 setgray Solid {pop []} if 0 setdash} ifelse} def
/BL {stroke userlinewidth 2 mul setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
/AL {stroke userlinewidth 2 div setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
/UL {dup gnulinewidth mul /userlinewidth exch def
	dup 1 lt {pop 1} if 10 mul /udl exch def} def
/PL {stroke userlinewidth setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
% Default Line colors
/LCw {1 1 1} def
/LCb {0 0 0} def
/LCa {0 0 0} def
/LC0 {1 0 0} def
/LC1 {0 1 0} def
/LC2 {0 0 1} def
/LC3 {1 0 1} def
/LC4 {0 1 1} def
/LC5 {1 1 0} def
/LC6 {0 0 0} def
/LC7 {1 0.3 0} def
/LC8 {0.5 0.5 0.5} def
% Default Line Types
/LTw {PL [] 1 setgray} def
/LTb {BL [] LCb DL} def
/LTa {AL [1 udl mul 2 udl mul] 0 setdash LCa setrgbcolor} def
/LT0 {PL [] LC0 DL} def
/LT1 {PL [4 dl1 2 dl2] LC1 DL} def
/LT2 {PL [2 dl1 3 dl2] LC2 DL} def
/LT3 {PL [1 dl1 1.5 dl2] LC3 DL} def
/LT4 {PL [6 dl1 2 dl2 1 dl1 2 dl2] LC4 DL} def
/LT5 {PL [3 dl1 3 dl2 1 dl1 3 dl2] LC5 DL} def
/LT6 {PL [2 dl1 2 dl2 2 dl1 6 dl2] LC6 DL} def
/LT7 {PL [1 dl1 2 dl2 6 dl1 2 dl2 1 dl1 2 dl2] LC7 DL} def
/LT8 {PL [2 dl1 2 dl2 2 dl1 2 dl2 2 dl1 2 dl2 2 dl1 4 dl2] LC8 DL} def
/Pnt {stroke [] 0 setdash gsave 1 setlinecap M 0 0 V stroke grestore} def
/Dia {stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt} def
/Pls {stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
 } def
/Box {stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt} def
/Crs {stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke} def
/TriU {stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt} def
/Star {2 copy Pls Crs} def
/BoxF {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath fill} def
/TriUF {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill} def
/TriD {stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt} def
/TriDF {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill} def
/Pent {stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt} def
/PentF {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore} def
/Circle {stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt} def
/CircleF {stroke [] 0 setdash hpt 0 360 arc fill} def
/C0 {BL [] 0 setdash 2 copy moveto vpt 90 450 arc} bind def
/C1 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C2 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C3 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C4 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 180 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C5 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc
	2 copy moveto
	2 copy vpt 180 270 arc closepath fill
	vpt 0 360 arc} bind def
/C6 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C7 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C8 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 270 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C9 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 270 450 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C10 {BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
	2 copy moveto
	2 copy vpt 90 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C11 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 180 arc closepath fill
	2 copy moveto
	2 copy vpt 270 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C12 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 180 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C13 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc closepath fill
	2 copy moveto
	2 copy vpt 180 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C14 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 360 arc closepath fill
	vpt 0 360 arc} bind def
/C15 {BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/Rec {newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
	neg 0 rlineto closepath} bind def
/Square {dup Rec} bind def
/Bsquare {vpt sub exch vpt sub exch vpt2 Square} bind def
/S0 {BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare} bind def
/S1 {BL [] 0 setdash 2 copy vpt Square fill Bsquare} bind def
/S2 {BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare} bind def
/S3 {BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare} bind def
/S4 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare} bind def
/S5 {BL [] 0 setdash 2 copy 2 copy vpt Square fill
	exch vpt sub exch vpt sub vpt Square fill Bsquare} bind def
/S6 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare} bind def
/S7 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
	2 copy vpt Square fill Bsquare} bind def
/S8 {BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare} bind def
/S9 {BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare} bind def
/S10 {BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
	Bsquare} bind def
/S11 {BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
	Bsquare} bind def
/S12 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare} bind def
/S13 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
	2 copy vpt Square fill Bsquare} bind def
/S14 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
	2 copy exch vpt sub exch vpt Square fill Bsquare} bind def
/S15 {BL [] 0 setdash 2 copy Bsquare fill Bsquare} bind def
/D0 {gsave translate 45 rotate 0 0 S0 stroke grestore} bind def
/D1 {gsave translate 45 rotate 0 0 S1 stroke grestore} bind def
/D2 {gsave translate 45 rotate 0 0 S2 stroke grestore} bind def
/D3 {gsave translate 45 rotate 0 0 S3 stroke grestore} bind def
/D4 {gsave translate 45 rotate 0 0 S4 stroke grestore} bind def
/D5 {gsave translate 45 rotate 0 0 S5 stroke grestore} bind def
/D6 {gsave translate 45 rotate 0 0 S6 stroke grestore} bind def
/D7 {gsave translate 45 rotate 0 0 S7 stroke grestore} bind def
/D8 {gsave translate 45 rotate 0 0 S8 stroke grestore} bind def
/D9 {gsave translate 45 rotate 0 0 S9 stroke grestore} bind def
/D10 {gsave translate 45 rotate 0 0 S10 stroke grestore} bind def
/D11 {gsave translate 45 rotate 0 0 S11 stroke grestore} bind def
/D12 {gsave translate 45 rotate 0 0 S12 stroke grestore} bind def
/D13 {gsave translate 45 rotate 0 0 S13 stroke grestore} bind def
/D14 {gsave translate 45 rotate 0 0 S14 stroke grestore} bind def
/D15 {gsave translate 45 rotate 0 0 S15 stroke grestore} bind def
/DiaE {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke} def
/BoxE {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke} def
/TriUE {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke} def
/TriDE {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke} def
/PentE {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore} def
/CircE {stroke [] 0 setdash 
  hpt 0 360 arc stroke} def
/Opaque {gsave closepath 1 setgray fill grestore 0 setgray closepath} def
/DiaW {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke} def
/BoxW {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke} def
/TriUW {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke} def
/TriDW {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke} def
/PentW {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore} def
/CircW {stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke} def
/BoxFill {gsave Rec 1 setgray fill grestore} def
/Density {
  /Fillden exch def
  currentrgbcolor
  /ColB exch def /ColG exch def /ColR exch def
  /ColR ColR Fillden mul Fillden sub 1 add def
  /ColG ColG Fillden mul Fillden sub 1 add def
  /ColB ColB Fillden mul Fillden sub 1 add def
  ColR ColG ColB setrgbcolor} def
/BoxColFill {gsave Rec PolyFill} def
/PolyFill {gsave Density fill grestore grestore} def
/h {rlineto rlineto rlineto gsave closepath fill grestore} bind def
%
% PostScript Level 1 Pattern Fill routine for rectangles
% Usage: x y w h s a XX PatternFill
%	x,y = lower left corner of box to be filled
%	w,h = width and height of box
%	  a = angle in degrees between lines and x-axis
%	 XX = 0/1 for no/yes cross-hatch
%
/PatternFill {gsave /PFa [ 9 2 roll ] def
  PFa 0 get PFa 2 get 2 div add PFa 1 get PFa 3 get 2 div add translate
  PFa 2 get -2 div PFa 3 get -2 div PFa 2 get PFa 3 get Rec
  gsave 1 setgray fill grestore clip
  currentlinewidth 0.5 mul setlinewidth
  /PFs PFa 2 get dup mul PFa 3 get dup mul add sqrt def
  0 0 M PFa 5 get rotate PFs -2 div dup translate
  0 1 PFs PFa 4 get div 1 add floor cvi
	{PFa 4 get mul 0 M 0 PFs V} for
  0 PFa 6 get ne {
	0 1 PFs PFa 4 get div 1 add floor cvi
	{PFa 4 get mul 0 2 1 roll M PFs 0 V} for
 } if
  stroke grestore} def
%
/languagelevel where
 {pop languagelevel} {1} ifelse
 2 lt
	{/InterpretLevel1 true def}
	{/InterpretLevel1 Level1 def}
 ifelse
%
% PostScript level 2 pattern fill definitions
%
/Level2PatternFill {
/Tile8x8 {/PaintType 2 /PatternType 1 /TilingType 1 /BBox [0 0 8 8] /XStep 8 /YStep 8}
	bind def
/KeepColor {currentrgbcolor [/Pattern /DeviceRGB] setcolorspace} bind def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 8 8 L 0 8 M 8 0 L stroke} 
>> matrix makepattern
/Pat1 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 8 8 L 0 8 M 8 0 L stroke
	0 4 M 4 8 L 8 4 L 4 0 L 0 4 L stroke}
>> matrix makepattern
/Pat2 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 0 8 L
	8 8 L 8 0 L 0 0 L fill}
>> matrix makepattern
/Pat3 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -4 8 M 8 -4 L
	0 12 M 12 0 L stroke}
>> matrix makepattern
/Pat4 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -4 0 M 8 12 L
	0 -4 M 12 8 L stroke}
>> matrix makepattern
/Pat5 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -2 8 M 4 -4 L
	0 12 M 8 -4 L 4 12 M 10 0 L stroke}
>> matrix makepattern
/Pat6 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -2 0 M 4 12 L
	0 -4 M 8 12 L 4 -4 M 10 8 L stroke}
>> matrix makepattern
/Pat7 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 8 -2 M -4 4 L
	12 0 M -4 8 L 12 4 M 0 10 L stroke}
>> matrix makepattern
/Pat8 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 -2 M 12 4 L
	-4 0 M 12 8 L -4 4 M 8 10 L stroke}
>> matrix makepattern
/Pat9 exch def
/Pattern1 {PatternBgnd KeepColor Pat1 setpattern} bind def
/Pattern2 {PatternBgnd KeepColor Pat2 setpattern} bind def
/Pattern3 {PatternBgnd KeepColor Pat3 setpattern} bind def
/Pattern4 {PatternBgnd KeepColor Landscape {Pat5} {Pat4} ifelse setpattern} bind def
/Pattern5 {PatternBgnd KeepColor Landscape {Pat4} {Pat5} ifelse setpattern} bind def
/Pattern6 {PatternBgnd KeepColor Landscape {Pat9} {Pat6} ifelse setpattern} bind def
/Pattern7 {PatternBgnd KeepColor Landscape {Pat8} {Pat7} ifelse setpattern} bind def
} def
%
%
%End of PostScript Level 2 code
%
/PatternBgnd {
  TransparentPatterns {} {gsave 1 setgray fill grestore} ifelse
} def
%
% Substitute for Level 2 pattern fill codes with
% grayscale if Level 2 support is not selected.
%
/Level1PatternFill {
/Pattern1 {0.250 Density} bind def
/Pattern2 {0.500 Density} bind def
/Pattern3 {0.750 Density} bind def
/Pattern4 {0.125 Density} bind def
/Pattern5 {0.375 Density} bind def
/Pattern6 {0.625 Density} bind def
/Pattern7 {0.875 Density} bind def
} def
%
% Now test for support of Level 2 code
%
Level1 {Level1PatternFill} {Level2PatternFill} ifelse
%
/Symbol-Oblique /Symbol findfont [1 0 .167 1 0 0] makefont
dup length dict begin {1 index /FID eq {pop pop} {def} ifelse} forall
currentdict end definefont pop
Level1 SuppressPDFMark or 
{} {
/SDict 10 dict def
systemdict /pdfmark known not {
  userdict /pdfmark systemdict /cleartomark get put
} if
SDict begin [
  /Title (bath_nr3.tex)
  /Subject (gnuplot plot)
  /Creator (gnuplot 4.5 patchlevel 0)
  /Author (Matt)
%  /Producer (gnuplot)
%  /Keywords ()
  /CreationDate (Sun Sep 04 20:15:10 2011)
  /DOCINFO pdfmark
end
} ifelse
end
%%EndProlog
gnudict begin
gsave
doclip
0 0 translate
0.050 0.050 scale
0 setgray
newpath
1.000 UL
LTb
1.000 UP
1.000 UL
LTb
1.000 UL
LT0
LCa setrgbcolor
1.000 UL
LT0
LCa setrgbcolor
gsave 2115 1386 N -1 8 V 0 9 V -2 8 V -1 9 V -2 8 V -3 8 V -2 9 V -4 8 V -3 7 V -5 8 V -4 7 V -5 7 V -5 7 V -6 7 V -6 6 V -6 6 V -7 6 V -7 5 V -7 5 V -7 4 V -8 5 V -7 3 V -8 4 V -9 2 V -8 3 V -8 2 V -9 1 V -8 2 V -9 0 V -8 1 V -9 -1 V -9 0 V -8 -2 V -9 -1 V -8 -2 V -8 -3 V -9 -2 V -8 -4 V -7 -3 V -8 -5 V -7 -4 V -7 -5 V -7 -5 V -7 -6 V -6 -6 V -6 -6 V -6 -7 V -5 -7 V -5 -7 V -4 -7 V -5 -8 V -3 -7 V -4 -8 V -2 -9 V -3 -8 V -2 -8 V -1 -9 V -2 -8 V 0 -9 V 0 -8 V 0 -9 V 0 -9 V 2 -8 V 1 -9 V 2 -8 V 3 -8 V 2 -9 V 4 -8 V 3 -7 V 5 -8 V 4 -7 V 5 -7 V 5 -7 V 6 -7 V 6 -6 V 6 -6 V 7 -6 V 7 -5 V 7 -5 V 7 -4 V 8 -5 V 7 -3 V 8 -4 V 9 -2 V 8 -3 V 8 -2 V 9 -1 V 8 -2 V 9 0 V 8 0 V 9 0 V 9 0 V 8 2 V 9 1 V 8 2 V 8 3 V 9 2 V 8 4 V 7 3 V 8 5 V 7 4 V 7 5 V 7 5 V 7 6 V 2066 1269 L 6 6 V 6 7 V 5 7 V 5 7 V 4 7 V 5 8 V 3 7 V 4 8 V 2 9 V 3 8 V 2 8 V 1 9 V 2 8 V 0 9 V 1 8 V 1 PolyFill
2115 1386 M
-1 8 V
0 9 V
-2 8 V
-1 9 V
-2 8 V
-3 8 V
-2 9 V
-4 8 V
-3 7 V
-5 8 V
-4 7 V
-5 7 V
-5 7 V
-6 7 V
-6 6 V
-6 6 V
-7 6 V
-7 5 V
-7 5 V
-7 4 V
-8 5 V
-7 3 V
-8 4 V
-9 2 V
-8 3 V
-8 2 V
-9 1 V
-8 2 V
-9 0 V
-8 1 V
-9 -1 V
-9 0 V
-8 -2 V
-9 -1 V
-8 -2 V
-8 -3 V
-9 -2 V
-8 -4 V
-7 -3 V
-8 -5 V
-7 -4 V
-7 -5 V
-7 -5 V
-7 -6 V
-6 -6 V
-6 -6 V
-6 -7 V
-5 -7 V
-5 -7 V
-4 -7 V
-5 -8 V
-3 -7 V
-4 -8 V
-2 -9 V
-3 -8 V
-2 -8 V
-1 -9 V
-2 -8 V
0 -9 V
0 -8 V
0 -9 V
0 -9 V
2 -8 V
1 -9 V
2 -8 V
3 -8 V
2 -9 V
4 -8 V
3 -7 V
5 -8 V
4 -7 V
5 -7 V
5 -7 V
6 -7 V
6 -6 V
6 -6 V
7 -6 V
7 -5 V
7 -5 V
7 -4 V
8 -5 V
7 -3 V
8 -4 V
9 -2 V
8 -3 V
8 -2 V
9 -1 V
8 -2 V
9 0 V
8 0 V
9 0 V
9 0 V
8 2 V
9 1 V
8 2 V
8 3 V
9 2 V
8 4 V
7 3 V
8 5 V
7 4 V
7 5 V
7 5 V
7 6 V
stroke 2060 1263 M
6 6 V
6 6 V
6 7 V
5 7 V
5 7 V
4 7 V
5 8 V
3 7 V
4 8 V
2 9 V
3 8 V
2 8 V
1 9 V
2 8 V
0 9 V
1 8 V
stroke
3.000 UL
LTb
LCa setrgbcolor
3.000 UL
LTb
LCa setrgbcolor
2396 791 M
-4 18 V
-4 -18 V
4 -15 R
0 33 V
stroke
gsave [] 0 setdash
2396 791 M
-4 18 V
-4 -18 V
stroke
grestore
965 526 M
-4 18 V
-4 -18 V
4 -11 R
0 29 V
stroke
gsave [] 0 setdash
965 526 M
-4 18 V
-4 -18 V
stroke
grestore
816 686 M
6 -26 V
6 26 V
-6 64 R
0 -90 V
stroke
gsave [] 0 setdash
816 686 M
6 -26 V
6 26 V
stroke
grestore
3241 2085 M
-4 18 V
-4 -18 V
4 4 R
0 14 V
stroke
gsave [] 0 setdash
3241 2085 M
-4 18 V
-4 -18 V
stroke
grestore
2333 2231 M
7 -28 V
7 28 V
-7 71 R
0 -99 V
stroke
gsave [] 0 setdash
2333 2231 M
7 -28 V
7 28 V
stroke
grestore
3021 2259 M
-4 18 V
-4 -18 V
4 -5 R
0 23 V
stroke
gsave [] 0 setdash
3021 2259 M
-4 18 V
-4 -18 V
stroke
grestore
796 2479 M
0 52 V
599 -779 R
4 -18 V
4 18 V
-4 31 R
0 -49 V
stroke
gsave [] 0 setdash
1395 1752 M
4 -18 V
4 18 V
stroke
grestore
3319 2124 M
9 -36 V
9 36 V
-9 91 R
0 -127 V
stroke
gsave [] 0 setdash
3319 2124 M
9 -36 V
9 36 V
stroke
grestore
2414 646 M
4 -18 V
4 18 V
-4 3 R
0 -21 V
stroke
gsave [] 0 setdash
2414 646 M
4 -18 V
4 18 V
stroke
grestore
2513 327 M
11 -42 V
11 42 V
-11 103 R
0 -145 V
stroke
gsave [] 0 setdash
2513 327 M
11 -42 V
11 42 V
stroke
grestore
2972 1907 M
4 -18 V
4 18 V
-4 9 R
0 -27 V
stroke
gsave [] 0 setdash
2972 1907 M
4 -18 V
4 18 V
stroke
grestore
403 1074 M
4 -18 V
4 18 V
-4 -8 R
0 -10 V
stroke
gsave [] 0 setdash
403 1074 M
4 -18 V
4 18 V
stroke
grestore
565 2132 M
-4 18 V
-4 -18 V
4 -2 R
0 20 V
stroke
gsave [] 0 setdash
565 2132 M
-4 18 V
-4 -18 V
stroke
grestore
2206 1838 M
-4 18 V
-4 -18 V
4 1 R
0 17 V
stroke
gsave [] 0 setdash
2206 1838 M
-4 18 V
-4 -18 V
stroke
grestore
1816 594 M
4 -18 V
4 18 V
-4 30 R
0 -48 V
stroke
gsave [] 0 setdash
1816 594 M
4 -18 V
4 18 V
stroke
grestore
665 923 M
5 -20 V
5 20 V
-5 52 R
0 -72 V
stroke
gsave [] 0 setdash
665 923 M
5 -20 V
5 20 V
stroke
grestore
3003 504 M
-4 18 V
-4 -18 V
4 -23 R
0 41 V
stroke
gsave [] 0 setdash
3003 504 M
-4 18 V
-4 -18 V
stroke
grestore
1920 2337 M
5 -20 V
5 20 V
-5 50 R
0 -70 V
stroke
gsave [] 0 setdash
1920 2337 M
5 -20 V
5 20 V
stroke
grestore
2395 1249 M
5 -19 V
5 19 V
-5 50 R
0 -69 V
stroke
gsave [] 0 setdash
2395 1249 M
5 -19 V
5 19 V
stroke
grestore
2238 944 M
5 -20 V
5 20 V
-5 52 R
0 -72 V
stroke
gsave [] 0 setdash
2238 944 M
5 -20 V
5 20 V
stroke
grestore
2117 1185 M
-4 18 V
-4 -18 V
4 8 R
0 10 V
stroke
gsave [] 0 setdash
2117 1185 M
-4 18 V
-4 -18 V
stroke
grestore
1381 1003 M
-7 28 V
-7 -28 V
7 -69 R
0 97 V
stroke
gsave [] 0 setdash
1381 1003 M
-7 28 V
-7 -28 V
stroke
grestore
1601 2008 M
7 -28 V
7 28 V
-7 72 R
0 -100 V
stroke
gsave [] 0 setdash
1601 2008 M
7 -28 V
7 28 V
stroke
grestore
1330 468 M
-4 18 V
-4 -18 V
4 17 R
0 1 V
stroke
gsave [] 0 setdash
1330 468 M
-4 18 V
-4 -18 V
stroke
grestore
1547 2378 M
-4 18 V
-4 -18 V
4 -26 R
0 44 V
stroke
gsave [] 0 setdash
1547 2378 M
-4 18 V
-4 -18 V
stroke
grestore
2464 1092 M
-6 23 V
-6 -23 V
6 -59 R
0 82 V
stroke
gsave [] 0 setdash
2464 1092 M
-6 23 V
-6 -23 V
stroke
grestore
3014 319 M
-6 24 V
-6 -24 V
6 -59 R
0 83 V
stroke
gsave [] 0 setdash
3014 319 M
-6 24 V
-6 -24 V
stroke
grestore
797 1547 M
-4 18 V
-4 -18 V
4 -18 R
0 36 V
stroke
gsave [] 0 setdash
797 1547 M
-4 18 V
-4 -18 V
stroke
grestore
1452 2102 M
4 -18 V
4 18 V
-4 42 R
0 -60 V
stroke
gsave [] 0 setdash
1452 2102 M
4 -18 V
4 18 V
stroke
grestore
1213 2273 M
4 -18 V
4 18 V
-4 22 R
0 -40 V
stroke
gsave [] 0 setdash
1213 2273 M
4 -18 V
4 18 V
stroke
grestore
3196 2066 M
-4 18 V
-4 -18 V
4 17 R
0 1 V
stroke
gsave [] 0 setdash
3196 2066 M
-4 18 V
-4 -18 V
stroke
grestore
2080 274 M
6 -23 V
6 23 V
-6 57 R
0 -80 V
stroke
gsave [] 0 setdash
2080 274 M
6 -23 V
6 23 V
stroke
grestore
612 1052 M
6 -26 V
6 26 V
-6 64 R
0 -90 V
stroke
gsave [] 0 setdash
612 1052 M
6 -26 V
6 26 V
stroke
grestore
2377 1895 M
-4 18 V
-4 -18 V
4 -24 R
0 42 V
stroke
gsave [] 0 setdash
2377 1895 M
-4 18 V
-4 -18 V
stroke
grestore
484 2148 M
-8 33 V
-8 -33 V
8 -82 R
0 115 V
stroke
gsave [] 0 setdash
484 2148 M
-8 33 V
-8 -33 V
stroke
grestore
3414 2133 M
4 -18 V
4 18 V
-4 7 R
0 -25 V
stroke
gsave [] 0 setdash
3414 2133 M
4 -18 V
4 18 V
stroke
grestore
323 507 M
6 -24 V
6 24 V
-6 62 R
0 -86 V
stroke
gsave [] 0 setdash
323 507 M
6 -24 V
6 24 V
stroke
grestore
1156 2356 M
-10 37 V
-10 -37 V
10 -94 R
0 131 V
stroke
gsave [] 0 setdash
1156 2356 M
-10 37 V
-10 -37 V
stroke
grestore
1883 2504 M
4 -18 V
4 18 V
-4 5 R
0 -23 V
stroke
gsave [] 0 setdash
1883 2504 M
4 -18 V
4 18 V
stroke
grestore
2513 1621 M
-11 43 V
-11 -43 V
11 -108 R
0 151 V
stroke
gsave [] 0 setdash
2513 1621 M
-11 43 V
-11 -43 V
stroke
grestore
3519 1868 M
4 -18 V
4 18 V
-4 -17 R
0 -1 V
stroke
gsave [] 0 setdash
3519 1868 M
4 -18 V
4 18 V
stroke
grestore
705 2185 M
-4 18 V
-4 -18 V
4 -6 R
0 24 V
stroke
gsave [] 0 setdash
705 2185 M
-4 18 V
-4 -18 V
stroke
grestore
2791 673 M
4 -18 V
4 18 V
-4 -10 R
0 -8 V
stroke
gsave [] 0 setdash
2791 673 M
4 -18 V
4 18 V
stroke
grestore
437 1441 M
stroke
gsave [] 0 setdash
grestore
677 1068 M
-4 18 V
-4 -18 V
4 5 R
0 13 V
stroke
gsave [] 0 setdash
677 1068 M
-4 18 V
-4 -18 V
stroke
grestore
3265 1068 M
-4 18 V
-4 -18 V
4 -36 R
0 54 V
stroke
gsave [] 0 setdash
3265 1068 M
-4 18 V
-4 -18 V
stroke
grestore
933 462 M
-4 18 V
-4 -18 V
4 14 R
0 4 V
stroke
gsave [] 0 setdash
933 462 M
-4 18 V
-4 -18 V
stroke
grestore
1676 1708 M
-4 18 V
-4 -18 V
4 -33 R
0 51 V
stroke
gsave [] 0 setdash
1676 1708 M
-4 18 V
-4 -18 V
stroke
grestore
1788 2271 M
7 -28 V
7 28 V
-7 72 R
0 -100 V
stroke
gsave [] 0 setdash
1788 2271 M
7 -28 V
7 28 V
stroke
grestore
336 638 M
4 -18 V
4 18 V
-4 4 R
0 -22 V
stroke
gsave [] 0 setdash
336 638 M
4 -18 V
4 18 V
stroke
grestore
2628 1690 M
-9 34 V
-9 -34 V
9 -86 R
0 120 V
stroke
gsave [] 0 setdash
2628 1690 M
-9 34 V
-9 -34 V
stroke
grestore
3358 2252 M
4 -18 V
4 18 V
-4 36 R
0 -54 V
stroke
gsave [] 0 setdash
3358 2252 M
4 -18 V
4 18 V
stroke
grestore
601 489 M
4 -18 V
4 18 V
-4 -3 R
0 -15 V
stroke
gsave [] 0 setdash
601 489 M
4 -18 V
4 18 V
stroke
grestore
2440 401 M
-4 18 V
-4 -18 V
4 -2 R
0 20 V
stroke
gsave [] 0 setdash
2440 401 M
-4 18 V
-4 -18 V
stroke
grestore
531 1948 M
4 -18 V
4 18 V
-4 16 R
0 -34 V
stroke
gsave [] 0 setdash
531 1948 M
4 -18 V
4 18 V
stroke
grestore
2043 881 M
5 -19 V
5 19 V
-5 47 R
0 -66 V
stroke
gsave [] 0 setdash
2043 881 M
5 -19 V
5 19 V
stroke
grestore
2723 2207 M
4 -18 V
4 18 V
-4 2 R
0 -20 V
stroke
gsave [] 0 setdash
2723 2207 M
4 -18 V
4 18 V
stroke
grestore
1648 1512 M
-4 18 V
-4 -18 V
4 13 R
0 5 V
stroke
gsave [] 0 setdash
1648 1512 M
-4 18 V
-4 -18 V
stroke
grestore
2831 932 M
-4 18 V
-4 -18 V
4 -45 R
0 63 V
stroke
gsave [] 0 setdash
2831 932 M
-4 18 V
-4 -18 V
stroke
grestore
1064 2292 M
4 -18 V
4 18 V
-4 -2 R
0 -16 V
stroke
gsave [] 0 setdash
1064 2292 M
4 -18 V
4 18 V
stroke
grestore
694 2288 M
-4 18 V
-4 -18 V
4 -12 R
0 30 V
stroke
gsave [] 0 setdash
694 2288 M
-4 18 V
-4 -18 V
stroke
grestore
3218 670 M
-4 18 V
-4 -18 V
4 -44 R
0 62 V
stroke
gsave [] 0 setdash
3218 670 M
-4 18 V
-4 -18 V
stroke
grestore
568 2493 M
4 -18 V
4 18 V
-4 21 R
0 -39 V
stroke
gsave [] 0 setdash
568 2493 M
4 -18 V
4 18 V
stroke
grestore
451 2240 M
-4 18 V
-4 -18 V
4 -1 R
0 19 V
stroke
gsave [] 0 setdash
451 2240 M
-4 18 V
-4 -18 V
stroke
grestore
1215 1981 M
-4 18 V
-4 -18 V
4 11 R
0 7 V
stroke
gsave [] 0 setdash
1215 1981 M
-4 18 V
-4 -18 V
stroke
grestore
3039 2032 M
-8 31 V
-8 -31 V
8 -78 R
0 109 V
stroke
gsave [] 0 setdash
3039 2032 M
-8 31 V
-8 -31 V
stroke
grestore
2906 1928 M
-5 21 V
-5 -21 V
5 -52 R
0 73 V
stroke
gsave [] 0 setdash
2906 1928 M
-5 21 V
-5 -21 V
stroke
grestore
2154 1776 M
stroke
gsave [] 0 setdash
grestore
738 386 M
-6 25 V
-6 -25 V
6 -63 R
0 88 V
stroke
gsave [] 0 setdash
738 386 M
-6 25 V
-6 -25 V
stroke
grestore
821 1040 M
4 -18 V
4 18 V
-4 7 R
0 -25 V
stroke
gsave [] 0 setdash
821 1040 M
4 -18 V
4 18 V
stroke
grestore
344 1492 M
-6 22 V
-6 -22 V
6 -57 R
0 79 V
stroke
gsave [] 0 setdash
344 1492 M
-6 22 V
-6 -22 V
stroke
grestore
2586 1785 M
-4 18 V
-4 -18 V
4 6 R
0 12 V
stroke
gsave [] 0 setdash
2586 1785 M
-4 18 V
-4 -18 V
stroke
grestore
1469 1398 M
4 -18 V
4 18 V
-4 -3 R
0 -15 V
stroke
gsave [] 0 setdash
1469 1398 M
4 -18 V
4 18 V
stroke
grestore
2213 1574 M
-4 18 V
-4 -18 V
4 8 R
0 10 V
stroke
gsave [] 0 setdash
2213 1574 M
-4 18 V
-4 -18 V
stroke
grestore
1843 1795 M
-4 18 V
-4 -18 V
4 -41 R
0 59 V
stroke
gsave [] 0 setdash
1843 1795 M
-4 18 V
-4 -18 V
stroke
grestore
3575 763 M
4 -18 V
4 18 V
-4 26 R
0 -44 V
stroke
gsave [] 0 setdash
3575 763 M
4 -18 V
4 18 V
stroke
grestore
2198 2075 M
4 -18 V
4 18 V
-4 24 R
0 -42 V
stroke
gsave [] 0 setdash
2198 2075 M
4 -18 V
4 18 V
stroke
grestore
1708 1403 M
-4 18 V
-4 -18 V
4 -10 R
0 28 V
stroke
gsave [] 0 setdash
1708 1403 M
-4 18 V
-4 -18 V
stroke
grestore
2932 1170 M
8 -30 V
8 30 V
-8 76 R
0 -106 V
stroke
gsave [] 0 setdash
2932 1170 M
8 -30 V
8 30 V
stroke
grestore
3167 275 M
0 -35 V
411 1337 M
-5 19 V
-5 -19 V
5 -50 R
0 69 V
stroke
gsave [] 0 setdash
411 1337 M
-5 19 V
-5 -19 V
stroke
grestore
2042 978 M
4 -18 V
4 18 V
-4 19 R
0 -37 V
stroke
gsave [] 0 setdash
2042 978 M
4 -18 V
4 18 V
stroke
grestore
2843 1945 M
-7 27 V
-7 -27 V
7 -69 R
0 96 V
stroke
gsave [] 0 setdash
2843 1945 M
-7 27 V
-7 -27 V
stroke
grestore
1232 1910 M
-4 18 V
-4 -18 V
4 1 R
0 17 V
stroke
gsave [] 0 setdash
1232 1910 M
-4 18 V
-4 -18 V
stroke
grestore
1567 292 M
0 -52 V
542 1655 M
5 -22 V
5 22 V
-5 54 R
0 -76 V
stroke
gsave [] 0 setdash
542 1655 M
5 -22 V
5 22 V
stroke
grestore
3013 2304 M
-4 18 V
-4 -18 V
4 0 R
0 18 V
stroke
gsave [] 0 setdash
3013 2304 M
-4 18 V
-4 -18 V
stroke
grestore
3590 2019 M
7 -28 V
7 28 V
-7 71 R
0 -99 V
stroke
gsave [] 0 setdash
3590 2019 M
7 -28 V
7 28 V
stroke
grestore
1542 277 M
4 -18 V
4 18 V
-4 -9 R
0 -9 V
stroke
gsave [] 0 setdash
1542 277 M
4 -18 V
4 18 V
stroke
grestore
2226 1465 M
-4 18 V
-4 -18 V
4 -26 R
0 44 V
stroke
gsave [] 0 setdash
2226 1465 M
-4 18 V
-4 -18 V
stroke
grestore
696 2520 M
0 11 V
585 1211 M
-4 18 V
-4 -18 V
4 -12 R
0 30 V
stroke
gsave [] 0 setdash
585 1211 M
-4 18 V
-4 -18 V
stroke
grestore
2572 590 M
4 -18 V
4 18 V
-4 -8 R
0 -10 V
stroke
gsave [] 0 setdash
2572 590 M
4 -18 V
4 18 V
stroke
grestore
705 1486 M
-4 18 V
-4 -18 V
4 11 R
0 7 V
stroke
gsave [] 0 setdash
705 1486 M
-4 18 V
-4 -18 V
stroke
grestore
3536 962 M
-4 18 V
-4 -18 V
4 -44 R
0 62 V
stroke
gsave [] 0 setdash
3536 962 M
-4 18 V
-4 -18 V
stroke
grestore
1671 450 M
4 -18 V
4 18 V
-4 25 R
0 -43 V
stroke
gsave [] 0 setdash
1671 450 M
4 -18 V
4 18 V
stroke
grestore
2104 2400 M
4 -18 V
4 18 V
-4 16 R
0 -34 V
stroke
gsave [] 0 setdash
2104 2400 M
4 -18 V
4 18 V
stroke
grestore
1.000 UP
1.000 UL
LTb
stroke
grestore
end
showpage
  }}%
\endGNUPLOTpicture
\endgroup
\endinput


==> figs/bath_nr4.tex <==
% GNUPLOT: plain TeX with Postscript
\begingroup
\catcode`\@=11\relax
\def\GNUPLOTspecial{%
  \def\do##1{\catcode`##1=12\relax}\dospecials
  \catcode`\{=1\catcode`\}=2\catcode\%=14\relax\special}%
%
\expandafter\ifx\csname GNUPLOTpicture\endcsname\relax
  \csname newdimen\endcsname\GNUPLOTunit
  \gdef\GNUPLOTpicture(#1,#2){\vbox to#2\GNUPLOTunit\bgroup
    \def\put(##1,##2)##3{\unskip\raise##2\GNUPLOTunit
      \hbox to0pt{\kern##1\GNUPLOTunit ##3\hss}\ignorespaces}%
    \def\ljust##1{\vbox to0pt{\vss\hbox to0pt{##1\hss}\vss}}%
    \def\cjust##1{\vbox to0pt{\vss\hbox to0pt{\hss ##1\hss}\vss}}%
    \def\rjust##1{\vbox to0pt{\vss\hbox to0pt{\hss ##1}\vss}}%
    \def\stack##1{\let\\=\cr\tabskip=0pt\halign{\hfil ####\hfil\cr ##1\crcr}}%
    \def\lstack##1{\hbox to0pt{\vbox to0pt{\vss\stack{##1}}\hss}}%
    \def\cstack##1{\hbox to0pt{\hss\vbox to0pt{\vss\stack{##1}}\hss}}%
    \def\rstack##1{\hbox to0pt{\vbox to0pt{\stack{##1}\vss}\hss}}%
    \vss\hbox to#1\GNUPLOTunit\bgroup\ignorespaces}%
  \gdef\endGNUPLOTpicture{\hss\egroup\egroup}%
\fi
\GNUPLOTunit=0.0500bp
\GNUPLOTpicture(3960,2772)
  {\GNUPLOTspecial{"
%!PS-Adobe-2.0 EPSF-2.0
%%Title: bath_nr4.tex
%%Creator: gnuplot 4.5 patchlevel 0
%%CreationDate: Sun Sep 04 20:15:11 2011
%%DocumentFonts: 
%%BoundingBox: 0 0 198 138
%%EndComments
%%BeginProlog
/gnudict 256 dict def
gnudict begin
%
% The following true/false flags may be edited by hand if desired.
% The unit line width and grayscale image gamma correction may also be changed.
%
/Color true def
/Blacktext true def
/Solid false def
/Dashlength 1 def
/Landscape false def
/Level1 false def
/Rounded false def
/ClipToBoundingBox false def
/SuppressPDFMark false def
/TransparentPatterns false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/Gamma 1.0 def
%
/vshift -66 def
/dl1 {
  10.0 Dashlength mul mul
  Rounded { currentlinewidth 0.75 mul sub dup 0 le { pop 0.01 } if } if
} def
/dl2 {
  10.0 Dashlength mul mul
  Rounded { currentlinewidth 0.75 mul add } if
} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/doclip {
  ClipToBoundingBox {
    newpath 0 0 moveto 198 0 lineto 198 138 lineto 0 138 lineto closepath
    clip
  } if
} def
%
% Gnuplot Prolog Version 4.4 (January 2010)
%
%/SuppressPDFMark true def
%
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/N {newpath moveto} bind def
/Z {closepath} bind def
/C {setrgbcolor} bind def
/f {rlineto fill} bind def
/Gshow {show} def   % May be redefined later in the file to support UTF-8
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow {currentpoint stroke M 0 vshift R 
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/Rshow {currentpoint stroke M dup stringwidth pop neg vshift R
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/Cshow {currentpoint stroke M dup stringwidth pop -2 div vshift R 
	Blacktext {gsave 0 setgray show grestore} {show} ifelse} def
/UP {dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def} def
/DL {Color {setrgbcolor Solid {pop []} if 0 setdash}
 {pop pop pop 0 setgray Solid {pop []} if 0 setdash} ifelse} def
/BL {stroke userlinewidth 2 mul setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
/AL {stroke userlinewidth 2 div setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
/UL {dup gnulinewidth mul /userlinewidth exch def
	dup 1 lt {pop 1} if 10 mul /udl exch def} def
/PL {stroke userlinewidth setlinewidth
	Rounded {1 setlinejoin 1 setlinecap} if} def
% Default Line colors
/LCw {1 1 1} def
/LCb {0 0 0} def
/LCa {0 0 0} def
/LC0 {1 0 0} def
/LC1 {0 1 0} def
/LC2 {0 0 1} def
/LC3 {1 0 1} def
/LC4 {0 1 1} def
/LC5 {1 1 0} def
/LC6 {0 0 0} def
/LC7 {1 0.3 0} def
/LC8 {0.5 0.5 0.5} def
% Default Line Types
/LTw {PL [] 1 setgray} def
/LTb {BL [] LCb DL} def
/LTa {AL [1 udl mul 2 udl mul] 0 setdash LCa setrgbcolor} def
/LT0 {PL [] LC0 DL} def
/LT1 {PL [4 dl1 2 dl2] LC1 DL} def
/LT2 {PL [2 dl1 3 dl2] LC2 DL} def
/LT3 {PL [1 dl1 1.5 dl2] LC3 DL} def
/LT4 {PL [6 dl1 2 dl2 1 dl1 2 dl2] LC4 DL} def
/LT5 {PL [3 dl1 3 dl2 1 dl1 3 dl2] LC5 DL} def
/LT6 {PL [2 dl1 2 dl2 2 dl1 6 dl2] LC6 DL} def
/LT7 {PL [1 dl1 2 dl2 6 dl1 2 dl2 1 dl1 2 dl2] LC7 DL} def
/LT8 {PL [2 dl1 2 dl2 2 dl1 2 dl2 2 dl1 2 dl2 2 dl1 4 dl2] LC8 DL} def
/Pnt {stroke [] 0 setdash gsave 1 setlinecap M 0 0 V stroke grestore} def
/Dia {stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt} def
/Pls {stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
 } def
/Box {stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt} def
/Crs {stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke} def
/TriU {stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt} def
/Star {2 copy Pls Crs} def
/BoxF {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath fill} def
/TriUF {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill} def
/TriD {stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt} def
/TriDF {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill} def
/Pent {stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt} def
/PentF {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore} def
/Circle {stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt} def
/CircleF {stroke [] 0 setdash hpt 0 360 arc fill} def
/C0 {BL [] 0 setdash 2 copy moveto vpt 90 450 arc} bind def
/C1 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C2 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C3 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C4 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 180 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C5 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc
	2 copy moveto
	2 copy vpt 180 270 arc closepath fill
	vpt 0 360 arc} bind def
/C6 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C7 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 270 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C8 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 270 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C9 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 270 450 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C10 {BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
	2 copy moveto
	2 copy vpt 90 180 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C11 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 180 arc closepath fill
	2 copy moveto
	2 copy vpt 270 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C12 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 180 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C13 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 0 90 arc closepath fill
	2 copy moveto
	2 copy vpt 180 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/C14 {BL [] 0 setdash 2 copy moveto
	2 copy vpt 90 360 arc closepath fill
	vpt 0 360 arc} bind def
/C15 {BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
	vpt 0 360 arc closepath} bind def
/Rec {newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
	neg 0 rlineto closepath} bind def
/Square {dup Rec} bind def
/Bsquare {vpt sub exch vpt sub exch vpt2 Square} bind def
/S0 {BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare} bind def
/S1 {BL [] 0 setdash 2 copy vpt Square fill Bsquare} bind def
/S2 {BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare} bind def
/S3 {BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare} bind def
/S4 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare} bind def
/S5 {BL [] 0 setdash 2 copy 2 copy vpt Square fill
	exch vpt sub exch vpt sub vpt Square fill Bsquare} bind def
/S6 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare} bind def
/S7 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
	2 copy vpt Square fill Bsquare} bind def
/S8 {BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare} bind def
/S9 {BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare} bind def
/S10 {BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
	Bsquare} bind def
/S11 {BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
	Bsquare} bind def
/S12 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare} bind def
/S13 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
	2 copy vpt Square fill Bsquare} bind def
/S14 {BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
	2 copy exch vpt sub exch vpt Square fill Bsquare} bind def
/S15 {BL [] 0 setdash 2 copy Bsquare fill Bsquare} bind def
/D0 {gsave translate 45 rotate 0 0 S0 stroke grestore} bind def
/D1 {gsave translate 45 rotate 0 0 S1 stroke grestore} bind def
/D2 {gsave translate 45 rotate 0 0 S2 stroke grestore} bind def
/D3 {gsave translate 45 rotate 0 0 S3 stroke grestore} bind def
/D4 {gsave translate 45 rotate 0 0 S4 stroke grestore} bind def
/D5 {gsave translate 45 rotate 0 0 S5 stroke grestore} bind def
/D6 {gsave translate 45 rotate 0 0 S6 stroke grestore} bind def
/D7 {gsave translate 45 rotate 0 0 S7 stroke grestore} bind def
/D8 {gsave translate 45 rotate 0 0 S8 stroke grestore} bind def
/D9 {gsave translate 45 rotate 0 0 S9 stroke grestore} bind def
/D10 {gsave translate 45 rotate 0 0 S10 stroke grestore} bind def
/D11 {gsave translate 45 rotate 0 0 S11 stroke grestore} bind def
/D12 {gsave translate 45 rotate 0 0 S12 stroke grestore} bind def
/D13 {gsave translate 45 rotate 0 0 S13 stroke grestore} bind def
/D14 {gsave translate 45 rotate 0 0 S14 stroke grestore} bind def
/D15 {gsave translate 45 rotate 0 0 S15 stroke grestore} bind def
/DiaE {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke} def
/BoxE {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke} def
/TriUE {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke} def
/TriDE {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke} def
/PentE {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore} def
/CircE {stroke [] 0 setdash 
  hpt 0 360 arc stroke} def
/Opaque {gsave closepath 1 setgray fill grestore 0 setgray closepath} def
/DiaW {stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke} def
/BoxW {stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke} def
/TriUW {stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke} def
/TriDW {stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke} def
/PentW {stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore} def
/CircW {stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke} def
/BoxFill {gsave Rec 1 setgray fill grestore} def
/Density {
  /Fillden exch def
  currentrgbcolor
  /ColB exch def /ColG exch def /ColR exch def
  /ColR ColR Fillden mul Fillden sub 1 add def
  /ColG ColG Fillden mul Fillden sub 1 add def
  /ColB ColB Fillden mul Fillden sub 1 add def
  ColR ColG ColB setrgbcolor} def
/BoxColFill {gsave Rec PolyFill} def
/PolyFill {gsave Density fill grestore grestore} def
/h {rlineto rlineto rlineto gsave closepath fill grestore} bind def
%
% PostScript Level 1 Pattern Fill routine for rectangles
% Usage: x y w h s a XX PatternFill
%	x,y = lower left corner of box to be filled
%	w,h = width and height of box
%	  a = angle in degrees between lines and x-axis
%	 XX = 0/1 for no/yes cross-hatch
%
/PatternFill {gsave /PFa [ 9 2 roll ] def
  PFa 0 get PFa 2 get 2 div add PFa 1 get PFa 3 get 2 div add translate
  PFa 2 get -2 div PFa 3 get -2 div PFa 2 get PFa 3 get Rec
  gsave 1 setgray fill grestore clip
  currentlinewidth 0.5 mul setlinewidth
  /PFs PFa 2 get dup mul PFa 3 get dup mul add sqrt def
  0 0 M PFa 5 get rotate PFs -2 div dup translate
  0 1 PFs PFa 4 get div 1 add floor cvi
	{PFa 4 get mul 0 M 0 PFs V} for
  0 PFa 6 get ne {
	0 1 PFs PFa 4 get div 1 add floor cvi
	{PFa 4 get mul 0 2 1 roll M PFs 0 V} for
 } if
  stroke grestore} def
%
/languagelevel where
 {pop languagelevel} {1} ifelse
 2 lt
	{/InterpretLevel1 true def}
	{/InterpretLevel1 Level1 def}
 ifelse
%
% PostScript level 2 pattern fill definitions
%
/Level2PatternFill {
/Tile8x8 {/PaintType 2 /PatternType 1 /TilingType 1 /BBox [0 0 8 8] /XStep 8 /YStep 8}
	bind def
/KeepColor {currentrgbcolor [/Pattern /DeviceRGB] setcolorspace} bind def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 8 8 L 0 8 M 8 0 L stroke} 
>> matrix makepattern
/Pat1 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 8 8 L 0 8 M 8 0 L stroke
	0 4 M 4 8 L 8 4 L 4 0 L 0 4 L stroke}
>> matrix makepattern
/Pat2 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 0 M 0 8 L
	8 8 L 8 0 L 0 0 L fill}
>> matrix makepattern
/Pat3 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -4 8 M 8 -4 L
	0 12 M 12 0 L stroke}
>> matrix makepattern
/Pat4 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -4 0 M 8 12 L
	0 -4 M 12 8 L stroke}
>> matrix makepattern
/Pat5 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -2 8 M 4 -4 L
	0 12 M 8 -4 L 4 12 M 10 0 L stroke}
>> matrix makepattern
/Pat6 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop -2 0 M 4 12 L
	0 -4 M 8 12 L 4 -4 M 10 8 L stroke}
>> matrix makepattern
/Pat7 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 8 -2 M -4 4 L
	12 0 M -4 8 L 12 4 M 0 10 L stroke}
>> matrix makepattern
/Pat8 exch def
<< Tile8x8
 /PaintProc {0.5 setlinewidth pop 0 -2 M 12 4 L
	-4 0 M 12 8 L -4 4 M 8 10 L stroke}
>> matrix makepattern
/Pat9 exch def
/Pattern1 {PatternBgnd KeepColor Pat1 setpattern} bind def
/Pattern2 {PatternBgnd KeepColor Pat2 setpattern} bind def
/Pattern3 {PatternBgnd KeepColor Pat3 setpattern} bind def
/Pattern4 {PatternBgnd KeepColor Landscape {Pat5} {Pat4} ifelse setpattern} bind def
/Pattern5 {PatternBgnd KeepColor Landscape {Pat4} {Pat5} ifelse setpattern} bind def
/Pattern6 {PatternBgnd KeepColor Landscape {Pat9} {Pat6} ifelse setpattern} bind def
/Pattern7 {PatternBgnd KeepColor Landscape {Pat8} {Pat7} ifelse setpattern} bind def
} def
%
%
%End of PostScript Level 2 code
%
/PatternBgnd {
  TransparentPatterns {} {gsave 1 setgray fill grestore} ifelse
} def
%
% Substitute for Level 2 pattern fill codes with
% grayscale if Level 2 support is not selected.
%
/Level1PatternFill {
/Pattern1 {0.250 Density} bind def
/Pattern2 {0.500 Density} bind def
/Pattern3 {0.750 Density} bind def
/Pattern4 {0.125 Density} bind def
/Pattern5 {0.375 Density} bind def
/Pattern6 {0.625 Density} bind def
/Pattern7 {0.875 Density} bind def
} def
%
% Now test for support of Level 2 code
%
Level1 {Level1PatternFill} {Level2PatternFill} ifelse
%
/Symbol-Oblique /Symbol findfont [1 0 .167 1 0 0] makefont
dup length dict begin {1 index /FID eq {pop pop} {def} ifelse} forall
currentdict end definefont pop
Level1 SuppressPDFMark or 
{} {
/SDict 10 dict def
systemdict /pdfmark known not {
  userdict /pdfmark systemdict /cleartomark get put
} if
SDict begin [
  /Title (bath_nr4.tex)
  /Subject (gnuplot plot)
  /Creator (gnuplot 4.5 patchlevel 0)
  /Author (Matt)
%  /Producer (gnuplot)
%  /Keywords ()
  /CreationDate (Sun Sep 04 20:15:11 2011)
  /DOCINFO pdfmark
end
} ifelse
end
%%EndProlog
gnudict begin
gsave
doclip
0 0 translate
0.050 0.050 scale
0 setgray
newpath
1.000 UL
LTb
1.000 UP
1.000 UL
LTb
1.000 UL
LT0
LCa setrgbcolor
1.000 UL
LT0
LCa setrgbcolor
gsave 2115 1386 N -1 8 V 0 9 V -2 8 V -1 9 V -2 8 V -3 8 V -2 9 V -4 8 V -3 7 V -5 8 V -4 7 V -5 7 V -5 7 V -6 7 V -6 6 V -6 6 V -7 6 V -7 5 V -7 5 V -7 4 V -8 5 V -7 3 V -8 4 V -9 2 V -8 3 V -8 2 V -9 1 V -8 2 V -9 0 V -8 1 V -9 -1 V -9 0 V -8 -2 V -9 -1 V -8 -2 V -8 -3 V -9 -2 V -8 -4 V -7 -3 V -8 -5 V -7 -4 V -7 -5 V -7 -5 V -7 -6 V -6 -6 V -6 -6 V -6 -7 V -5 -7 V -5 -7 V -4 -7 V -5 -8 V -3 -7 V -4 -8 V -2 -9 V -3 -8 V -2 -8 V -1 -9 V -2 -8 V 0 -9 V 0 -8 V 0 -9 V 0 -9 V 2 -8 V 1 -9 V 2 -8 V 3 -8 V 2 -9 V 4 -8 V 3 -7 V 5 -8 V 4 -7 V 5 -7 V 5 -7 V 6 -7 V 6 -6 V 6 -6 V 7 -6 V 7 -5 V 7 -5 V 7 -4 V 8 -5 V 7 -3 V 8 -4 V 9 -2 V 8 -3 V 8 -2 V 9 -1 V 8 -2 V 9 0 V 8 0 V 9 0 V 9 0 V 8 2 V 9 1 V 8 2 V 8 3 V 9 2 V 8 4 V 7 3 V 8 5 V 7 4 V 7 5 V 7 5 V 7 6 V 2066 1269 L 6 6 V 6 7 V 5 7 V 5 7 V 4 7 V 5 8 V 3 7 V 4 8 V 2 9 V 3 8 V 2 8 V 1 9 V 2 8 V 0 9 V 1 8 V 1 PolyFill
2115 1386 M
-1 8 V
0 9 V
-2 8 V
-1 9 V
-2 8 V
-3 8 V
-2 9 V
-4 8 V
-3 7 V
-5 8 V
-4 7 V
-5 7 V
-5 7 V
-6 7 V
-6 6 V
-6 6 V
-7 6 V
-7 5 V
-7 5 V
-7 4 V
-8 5 V
-7 3 V
-8 4 V
-9 2 V
-8 3 V
-8 2 V
-9 1 V
-8 2 V
-9 0 V
-8 1 V
-9 -1 V
-9 0 V
-8 -2 V
-9 -1 V
-8 -2 V
-8 -3 V
-9 -2 V
-8 -4 V
-7 -3 V
-8 -5 V
-7 -4 V
-7 -5 V
-7 -5 V
-7 -6 V
-6 -6 V
-6 -6 V
-6 -7 V
-5 -7 V
-5 -7 V
-4 -7 V
-5 -8 V
-3 -7 V
-4 -8 V
-2 -9 V
-3 -8 V
-2 -8 V
-1 -9 V
-2 -8 V
0 -9 V
0 -8 V
0 -9 V
0 -9 V
2 -8 V
1 -9 V
2 -8 V
3 -8 V
2 -9 V
4 -8 V
3 -7 V
5 -8 V
4 -7 V
5 -7 V
5 -7 V
6 -7 V
6 -6 V
6 -6 V
7 -6 V
7 -5 V
7 -5 V
7 -4 V
8 -5 V
7 -3 V
8 -4 V
9 -2 V
8 -3 V
8 -2 V
9 -1 V
8 -2 V
9 0 V
8 0 V
9 0 V
9 0 V
8 2 V
9 1 V
8 2 V
8 3 V
9 2 V
8 4 V
7 3 V
8 5 V
7 4 V
7 5 V
7 5 V
7 6 V
stroke 2060 1263 M
6 6 V
6 6 V
6 7 V
5 7 V
5 7 V
4 7 V
5 8 V
3 7 V
4 8 V
2 9 V
3 8 V
2 8 V
1 9 V
2 8 V
0 9 V
1 8 V
stroke
3.000 UL
LTb
3.000 UL
LTb
406 842 M
302 864 L
79 -71 V
619 703 M
302 864 L
stroke
gsave [] 0 setdash
406 842 M
302 864 L
79 -71 V
stroke
grestore
2780 1704 M
-17 -7 V
18 -2 V
24 8 R
-42 -6 V
stroke
gsave [] 0 setdash
2780 1704 M
-17 -7 V
18 -2 V
stroke
grestore
2931 1073 M
-15 -58 V
43 43 V
59 133 R
2916 1015 L
stroke
gsave [] 0 setdash
2931 1073 M
-15 -58 V
43 43 V
stroke
grestore
3430 1171 M
74 -10 V
-59 46 V
-173 51 R
232 -97 V
stroke
gsave [] 0 setdash
3430 1171 M
74 -10 V
-59 46 V
stroke
grestore
1241 2148 M
57 42 V
-71 -8 V
-151 -80 R
222 88 V
stroke
gsave [] 0 setdash
1241 2148 M
57 42 V
-71 -8 V
stroke
grestore
3071 1907 M
-22 27 V
5 -34 V
42 -74 R
-47 108 V
stroke
gsave [] 0 setdash
3071 1907 M
-22 27 V
5 -34 V
stroke
grestore
2121 1876 M
-48 24 V
29 -45 V
107 -77 R
-136 122 V
stroke
gsave [] 0 setdash
2121 1876 M
-48 24 V
29 -45 V
stroke
grestore
3158 485 M
-15 12 V
6 -18 V
32 -35 R
-38 53 V
stroke
gsave [] 0 setdash
3158 485 M
-15 12 V
6 -18 V
stroke
grestore
505 1524 M
30 82 V
-67 -55 V
365 1368 M
170 238 V
stroke
gsave [] 0 setdash
505 1524 M
30 82 V
-67 -55 V
stroke
grestore
2077 1150 M
-33 -34 V
46 13 V
93 70 R
-139 -83 V
stroke
gsave [] 0 setdash
2077 1150 M
-33 -34 V
46 13 V
stroke
grestore
1798 1784 M
20 -39 V
2 44 V
-33 102 R
31 -146 V
stroke
gsave [] 0 setdash
1798 1784 M
20 -39 V
2 44 V
stroke
grestore
1973 2444 M
35 68 V
-65 -41 V
1834 2321 M
174 191 V
stroke
gsave [] 0 setdash
1973 2444 M
35 68 V
-65 -41 V
stroke
grestore
3393 874 M
-7 -52 V
32 41 V
37 120 R
3386 822 L
stroke
gsave [] 0 setdash
3393 874 M
-7 -52 V
32 41 V
stroke
grestore
2364 2388 M
12 22 V
-21 -13 V
-38 -48 R
59 61 V
stroke
gsave [] 0 setdash
2364 2388 M
12 22 V
-21 -13 V
stroke
grestore
3452 1794 M
147 -12 V
2417 2017 M
6 -17 V
3 18 V
-4 -4 R
1 -14 V
stroke
gsave [] 0 setdash
2417 2017 M
6 -17 V
3 18 V
stroke
grestore
1.000 UP
1.000 UL
LTb
stroke
grestore
end
showpage
  }}%
\endGNUPLOTpicture
\endgroup
\endinput

